Meaningful Causal Aggregation and Paradoxical Confounding

In aggregated variables the impact of interventions is typically ill-defined because different micro-realizations of the same macro-intervention can result in different changes of downstream macro-variables. We show that this ill-definedness of causality on aggregated variables can turn unconfounded causal relations into confounded ones and vice versa, depending on the respective micro-realization. We argue that it is practically infeasible to only use aggregated causal systems when we are free from this ill-definedness. Instead, we need to accept that macro causal relations are typically defined only with reference to the micro states. On the positive side, we show that cause-effect relations can be aggregated when the macro interventions are such that the distribution of micro states is the same as in the observational distribution; we term this natural macro interventions. We also discuss generalizations of this observation.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> main_paper_Version_15-Feb-23.tex <==
\section{Introduction}

Discussions on publicly relevant questions in  
economy, politics, and health typically refer to 
variables that are actually aggregations over a large number of 
components. For instance, quantities like {\it employment rate}, {\it voter participation} or {\it vaccination rate} are usually aggregations over business sectors or/and over  the whole population of a country or region. 
%Despite all concerns that more fine grained information would actually be needed to discuss how changes of these quantities affect others, it is unrealistic to entirely abstain from causal claims on the aggregated level. 
%In many physical systems or real-world applications, % detailed 
%measurements are aggregated to obtain a high-level understanding of the system under study.
% Typical discussions about causal relations in economics, ecology, epidemiology and many other topics
% refer to processes that are actually too complex for human understanding. Any communication and analysis thus requires  
% simple models with highly aggregated variables.  
%For example, if a retail company wants to reason about how its sales impacts its revenue, it is impossible for them to reason using the sales of each individual product, as there would be too many. Instead, they aggregate individual-level sales and revenue, and directly ask about effects of total sales on total revenue. 
Following the literature \citep{Chalupka2016MultiLevelCS,Rubenstein2017}, we will refer to the aggregated variables (e.g. `total sales' and 'total revenue`of a company) as \textit{macro-variables}, and the detailed individual level quantities as \textit{micro-variables}. 

Previous works such as \citet{Rubenstein2017} and \citet{beckers19} show that macro variables do not necessarily preserve causal relationships among the micro ones,
which explicitly confirms the concerns raised above. 
Although \citet{Rubenstein2017} provide a notion of consistency between macro- and micro-models, their notion is strong since it requires that all microscopic realizations of
an intervention on an aggregated variable results in the same effect on aggregated downstream variables. 
%In particular, when many interventions on the micro-model can lead to the same intervention on the macro-level, their notion requires that all these interventions lead to the same effect on the macro level. 
As follow-up work, \citep{beckers19} proposes a sequence of definitions of causal consistency, starting from that of \citep{Rubenstein2017}, each new definition they provide is stronger than the previous.

These notions can be hard to satisfy in real world. If the retail company decides to increase its total sales (i.e. the sum over all different products) to $\bar{X}$, then there are multiple ways to do that. For example, they could sell $\bar{X}$ number of most expensive items, or they could sell $\bar{X}$ number of cheapest items, or anything in between. The total revenue will differ depending on their exact method of achieving total sales of $\bar{X}$, and thus by the notions of \citet{Rubenstein2017, beckers19} this aggregation is not consistent. In Example~\ref{ex:violate_rw17} we illustrate this with a formal example. 
% \kailash{\citept{Rubenstein2017} provide a general condition under which two structural equation models at different levels of detail are consistent. For example, a macro model admits a causal interpretation when they are averages of unconfounded micro variables that admit a linear SCM. (Maybe we can relate their exact transformation to confounding-inhibiting intervention?) In this work, we study the confounding property of macro-level variables when micro-variables are either confounded or unconfounded. \citept{Rubenstein2017} deals with the consistency of two data generating models\citep{Rubenstein2017}, whereas this work deals with the ``confounding-inhibiting'' or ``confounding-inducing'' property of macro variables resulting from coarse-graining. Contrasting \citept{Rubenstein2017} w.r.t. the strength of assumptions and applicability seems odd.}

Despite the difficulty of consistent aggregation in the real world, the concept of aggregation is ubiquitous. For example, economists study the impact of Gross Domestic Product on civil conflict \citep{Miguel2004EconomicSA} as it would be overwhelming to model each person's socioeconomic and political activities; 
% gene micro-array data often need to be aggregated to act as causes for diseases; 
physicists study the impact of pressure and temperature of gas inside a container because it is practically impossible to model the motions of individual particles. Thus, instead of asking whether there is an aggregation that is consistent in the sense
of  \citet{Rubenstein2017, beckers19}, we discuss how to make causal claims {\it relative to a class of micro realizations} of interventions on macro-variables.  
%the micro and macro models are consistent, we seek to understand their properties when they may not be consistent.  
% In particular, examples of questions we ask include: is the macro model always confounded when the micro model is confounded? 

% Despite the difficulty of consistent aggregation, it is nonetheless prevalent in practice. 

% Nevertheless, practitioners still go ahead and aggregate despite the difficulty of consistency. Because the definition of macro-variables in real-world systems is usually guided by simplicity and interpretability rather than consistency requirements. 

% Instead of asking for consistency, we ask to exploit \textit{heterogeneity} of micro-interventions that correspond to the same macro-intervention. 

We find that, as a result, \textit{confoundedness} is ambiguous in the macro-variables. 
% When the micro-variables are themselves unconfounded, confounding can actually arise from coarsening by choosing certain pairings of micro- and macro-interventions. 
%If micro-variables are themselves confounded, practitioners can actually remove confounding from the macro-variables by being deliberate in their choice of macro- and micro-intervention pairings, and \textit{vice versa}. We make precise the preceding statements in the paper, and we view this as a provocative result which challenges fields such as causal representation learning: is it after all possible to learn latent causal graphs when it is not well-defined? From a practical perspective, our result can be used to the advantage of the practitioners. For example, they may choose to use the intervention which promotes a sense of unconfoundedness in order to make effect inference easy. 
%\dominik{Leaning towards a different story line:} 
Rather than denying aggregation because of this ill-definedness, we argue that causal claims on the aggregated level can be valid relative to a notion of intervention that is to be specified. We will show that this view opens up the path to coarse-graining causal models that works under significantly weaker assumptions that those in the literature. 

% More generally speaking, we can ask under which conditions a graphical model of the statistical relations between
% macro-variables can be interpreted as a causal model {\it by defining interventions accordingly}. 

% \begin{figure*}[t]
%     \begin{minipage}{0.45\textwidth}
%       \begin{center}
%         \includegraphics[scale=0.45]{figures/sales_micromacro_1.pdf}
%       \end{center}
%     \end{minipage}
%     \begin{minipage}{0.45\textwidth}
%       \begin{center}
%         \includegraphics[scale=0.45]{figures/sales_micromacro_2.pdf}
%       \end{center}
%     \end{minipage}
%     \caption{Two different ways of realising the same intervention on $\bar{X}$. Note that we only see the difference in actual intervention in the micro-level because we are aware of the coarsening structure. If we are only aware of the macro-level without knowing that it comes from coarsening, we would conclude that both and left and right sides are the same intervention, which is clearly not true. \dominik{too large given the simplicity of this insight} }
%     \label{fig:sales_micromacro}
% \end{figure*}

% \dominik{a lot of space for such a simple thing, let's use a different scaling}

% \lipsum[1-4]%% On left column second page

% \begin{figure}[t]%% Put a picture that is too wide. It will continue in to the right column
%   \begin{minipage}[t]{0.65\linewidth}
%     \includegraphics[width=\linewidth]{figures/sales_micromacro_1.pdf}
%   \end{minipage}\rule{1em}{0pt}%
%   \begin{minipage}[t]{0.65\linewidth}
%     \includegraphics[width=\linewidth]{figures/sales_micromacro_2.pdf}
%   \end{minipage}
%   \caption{Two different ways of realising the same intervention on $\bar{X}$. Note that we only see the difference in actual intervention in the micro-level because we are aware of the coarsening structure. If we are only aware of the macro-level without knowing that it comes from coarsening, we would conclude that both and left and right sides are the same intervention, which is clearly not true.  }
%     \label{fig:sales_micromacro}
% \end{figure}

\begin{figure*}
\floatbox[{\capbeside\thisfloatsetup{capbesideposition={right,top},capbesidewidth=5cm,floatwidth=sidefil}}]{figure}
{\caption{Two different ways of realising the same intervention on $\bar{X}$. Note that we only see the difference in actual intervention in the micro-level because we are aware of the coarsening structure. If we are only aware of the macro-level without knowing that it comes from coarsening, we would conclude that both and left and right sides are the same intervention, which is clearly not true. }\label{fig:sales_micromacro}}
% {\includegraphics[width=5cm]{figures/sales_micromacro_1.pdf}}
  {\begin{minipage}[t]{0.47\linewidth}
    \includegraphics[width=\linewidth]{figures/sales_micromacro_1.pdf}
  \end{minipage}\rule{1em}{0pt}%
  \begin{minipage}[t]{0.47\linewidth}
    \includegraphics[width=\linewidth]{figures/sales_micromacro_2.pdf}
  \end{minipage}}
\vspace{-2.5ex}
\end{figure*}


Section~\ref{sec:formulation} introduces the framework under which we talk about micro- and macro-variable systems.
% We give definitions for micro- and macro-variables, coarsening map, macro intervention and macro confounding. 
In particular, we introduce the notions of \textit{confounding-inducing} and \textit{confounding-inhibiting} macro interventions, which formalise the idea of confoundedness arising from choices of interventions. Section~\ref{sec:unconfounded} discusses confounding resulting from aggregating unconfounded micro-models. We derive this phenomenon as a result of a change of coordinate systems. Section~\ref{sec:confounded} shows that even when micro models are themselves confounded, aggregated models can nevertheless sometimes be unconfounded. We focus on two specific settings: a general discrete setting and a continuous linear Gaussian setting. 
% We show that in both settings it can be possible to remove confounding by choosing the right intervention, i.e. the confounding-inhibiting macro intervention. 
% For the linear Gaussian setting, we provide an example for interpretation and discuss feasibility of confounding-inhibiting macro interventions when they exist.

%Finally, in Section~\ref{sec:conclusion}, we discuss related work and draw concluding remarks.

\section{Macro- and micro-intervention}\label{sec:formulation}

In this work, micro-level causal models are nothing but standard structural equation models, defined following the standard frameworks introduced by \citep{pearl09}. 
%and recast by \citep{peters_elements}. 
We in particular focus on \textit{acyclic} models. 

\begin{definition}[micro causal model]\label{def:micro}
A micro causal model is an acyclic structural causal model (SCM). 
%If $X$ is a causal parent of $Y$, this is graphically represented as
%\vspace{-4ex}
%\begin{figure}[H]
%    \centering
%	\begin{tikzpicture}[roundnode/.style={circle, draw=black!100, very thick, minimum size=0.5mm}, greynode/.style={circle, draw=black!100, fill=black!15, very thick, minimum size=0.5mm}, normalnode/.style={circle, draw=black!0, very thick, minimum size=0.5mm}, squarednode/.style={rectangle, draw=red!60, fill=red!5, very thick, minimum size=5mm}, arrowhead/.style={Triangle[length=3mm, width=2mm]}]
%		\node[roundnode] (x) at (-0.8,1) {$X$};
%		\node[roundnode] (y) at (0.8, 1) {$Y$};
%		\draw[-{Triangle[length=3mm, width=2mm]}, line width=1pt] (x) -- (y);
%	\end{tikzpicture}
%\end{figure}
%\vspace{-4ex}
%\end{definition}
%We follow \citep{pearl09} 
%and \citep{peters_elements} \dominik{could we avoid this self-citation?} 
%to define a structural causal model.
\begin{definition}[structural causal model]
A structural causal model (SCM) $M\defeq (\mathbf{S}, P_{\mathbf{N}})$ consists of a collection $\mathbf{S}$ of $d$ \textbf{(structural) assignments} 
\begin{align}
    X_j \defeq f_j(\text{\bf PA}_j, U_j), \;\; j=1,...,d,
\end{align}
where $\text{\bf PA}_j \subseteq \left\{X_1,\cdots, X_d\right\} \setminus \left\{X_j\right\}$ are called \textbf{parents of} $X_j$; and a joint distribution $P_{\mathbf{U}} = P_{U_1,\cdots, U_d}$ over the noise variables, which we require to be jointly independent; that is, $P_{\mathbf{U}}$ is a product distribution. We assume that the model is \textit{acyclic}, that is, no variable $X_j$ can be written as an assignment of itself by composition of structural assignments.
\end{definition}

Given a micro-causal model, macro-variables can be thought of to arise from applying an aggregation map on the micro-variables.
\begin{definition}[aggregation map, macro-variables]\label{def:coarsening}
Given a random variable $X$ with range $\cX$, an \textit{aggregation map} is a surjective but non-injective function $\pi: \cX \rightarrow \bar{\cX}$. Define $\bar{X} = \pi(X)$ to be the macro-variable of $X$ under $\pi$. 
\end{definition}
 Graphically, we represent the coarsening relationship by 
\dominik{people will be confused about the symmetric symbol. I know we had his discussion. What was the argument?}
%\vspace{-4ex}
\begin{figure}[H]
    \centering
	\begin{tikzpicture}[roundnode/.style={circle, draw=black!100, very thick, minimum size=0.5mm}, greynode/.style={circle, draw=black!100, fill=black!15, very thick, minimum size=0.5mm}, normalnode/.style={circle, draw=black!0, very thick, minimum size=0.5mm}, squarednode/.style={rectangle, draw=red!60, fill=red!5, very thick, minimum size=5mm}, arrowhead/.style={Triangle[length=3mm, width=2mm]}]
		\node[roundnode] (x) at (-0.8,1) {$X$};
		\node[roundnode] (xbar) at (0.8, 1) {$\bar{X}$};
		\draw[{Triangle[open, length=2mm, width=2mm]}-{Triangle[open, length=2mm, width=2mm]}] (x) -- (xbar);
	\end{tikzpicture}
\end{figure}
\vspace{-4ex}
We refer to this as the graph of $\pi$.

We will later consider separate coarsenings at each 
node. Then each $X_j$ will often be a vector in $\R^n$ and $\bar{X}_j$ the sum or average of all its components. 
Given a distribution $P(X_1,\dots,X_n)$ over the microvariables, defining $\pi_j$ for each node induces a joint distribution
$P(X_1,\dots,X_n,\pi(X_1,),\dots,\pi(X_n))$. 


%Then $\bar{X} \sim \pi_{\#} P$, the pushforward measure of $P$ under $\pi$. 



%In the case where $X$ is discrete, $\pi$ will map more than one value in $\cX$ to the same value in $\bar{\cX}$ i.e. $|\pi^{-1}(\bar{x})| > 1$ for some $\bar{x} \in \bar{X}$.
%\dominik{not only if its discrete}

\begin{definition}[amalgamated graph]
Given a micro causal model and a set of coarsening maps, we can define the amalgamated graph, $G^a\defeq (\cV, \bar{\cV}, \cE, \cC)$, where $V \in \cV$ if $V$ is a micro-variable, $\bar{V} \in \bar{\cV}$ if $\bar{V}$ is a macro-variable, $U\rightarrow V \in \cE$ if $U$ and $V$ are micro-variables and $U$ is a parent of $V$, and $S \leftrightarrow T \in \cC$ if $S$ is a micro-variable, $T$ is a macro-variable, and there is an aggregation map from $\cS$ to $\cT$.
\end{definition}

The first consequence of aggregation is that the aggregated variables may no longer form a causal model, as illustrated in the following:

\begin{example}\label{ex:violate_rw17}
For $j=1,2$, set $Y_j:=\alpha_j X_j$
$\bar{X}:=\pi_X(X_1,X_2)=X_1+X_2$, likewise 
$\bar{Y}:=\pi_Y(Y_1,Y_2)=Y_1+Y_2$.
Then, for $\alpha_1\neq \alpha_2$, the effect of setting $\bar{X}$ to $\bar{x}$ on $\bar{Y}$ is ill-defined without any further specification. 
%Let $M = (\mathbf{S}, P_{\mathbf{N}})$ be a micro causal model where 
%\begin{align*}
%    \mathbf{S} &= \left\{X_1 \defeq U_1, \; X_2 \defeq U_2, \; Y_1 \defeq \alpha_1 X_1, \; Y_2 \defeq \alpha_2 X_2\right\} 
%\end{align*}
%where $\alpha_1 \neq \alpha_2$, $\cU_1 = \{0, 1\}$, $\cU_2 = \{0,1\}$, $\text{supp}[P_{U_1}] = \text{supp}[P_{U_2}] = \{0,1\}$. Now, consider a set of interventions that we are interested in on the micro causal model.
%\begin{align*}
%    \cI = \{&i_1 = do(X_1\defeq 1, X_2 \defeq 0), \\&i_2 = do(X_1 \defeq 0, X_2 \defeq 1)\}.
%\end{align*}
%as well as aggregation maps $\bar{X}=\pi_X((X_1, X_2)) = X_1 + X_2$ and $\bar{Y} = \pi_Y((Y_1, Y_2)) = Y_1 + Y_2$. 

%Now applying $i_1$ to the system results in $X_1=1$, $X_2=0$, $Y_1=\alpha_1$, $Y_2=0$, and thus $\bar{X}=1$ and $\bar{Y}=\alpha_1$. Meanwhile, applying $i_2$ to the system results in $X_1 = 0$, $X_2 = 1$, $Y_1 = 0$, $Y_2 = \alpha_2$, and thus $\bar{X} = 1$ and $\bar{Y} = \alpha_2$. Thus, there is no structural assignment $f: \bar{\cX} \rightarrow \bar{\cY}$ s.t. 
%\begin{align*}
%    \pi_{\#} P^{do(i_k)} ( X_1, X_2, Y_1, Y_2) &= P^{do(\bar{X} \defeq 1)} (\bar{X}, \bar{Y})
%\end{align*}
%where $k = 1, 2$.

%Therefore, it is not possible to define a sensible causal model on the macro variables: since $X_1, X_2$ precede $Y_1, Y_2$ in causal order, $\bar{X}$ should also precede $\bar{Y}$ if there is a `macro causal model', yet there is no way to define a structural equation from $\bar{X}$ to $\bar{Y}$ that makes the `macro causal model' consistent with the micro model in the sense that the pushforward measure of interventions on the micro model is always equal to the interventional distribution on the macro model given by the corresponding intervention. Here, corresponding intervention is given by the aggregation map. The above intuition can be formalized - \citep{Rubenstein2017} provides a formal definition of consistency, which is violated by our example exactly for the reason we laid out. In fact, only when $\alpha_1 = \alpha_2$ are we able to obtain a consistent macro causal model under the definition of theirs. 
\end{example}

In reality, the case where $\alpha_1 = \alpha_2$ is rare, and the generic cases are when $\alpha_1 \neq \alpha_2$. So what shall we do then?
We propose to think of an intervention on the macro-variable \textit{in terms of} an intervention on the \textit{micro} level: since $X$ and $\bar{X}$ are connected via the map $\pi$, a change in $\bar{X}$ necessarily imposes a change on its preimage $\pi^{-1}(\bar{x})$. For example, if we sell 1000 more bottles of shampoo in total, this must reflect in the increase of sales for all individual shampoo brands. 

\begin{definition}[macro intervention]
A (stochastic)  \textit{macro-intervention}, $j$, is defined with respect to an aggregation map, $\pi$. It is a pair, $\left( do(\bar{X}\defeq \bar{x}), P^{do}_{\pi, \bar{x}}(X) \right)$, where $P^{do}_{\pi,\bar{x}}(X)$ is a probability measure over $\cX$ such that $\pi(x) = \bar{x}\;\; \forall x \in \text{supp}(P^{do}_{\pi,\bar{x}}(X))$. When it is clear in context which aggregation map we refer to, we simply write $P^{do}_{\bar{x}}(X)$ for light notation. 
\end{definition}
In order words, since the operation `setting $\bar{X}$ to $\bar{x}$' is not well-defined \textit{a priori}, its microscopic implementation needs to be specified whenever talking about it. 

Note, that there has been previous attempt in the literature which define interventions on the macro-variables in a similar way to us: \citet{Chalupka2016MultiLevelCS} also define a macro-level intervention via actual intervention on micro-variables.
\dominik{mention how they work with this definition any why they didn't solve our problem.}
Differing from their setting, we consider stochastic interventions~\citep{Correa_Bareinboim_2020} as well as deterministic, while they only consider the latter. 
% \kailash{todo: check if there is a better term)}
% \jonas{Maybe it is worth defining the set of allowed macro interventions. For example like 
% \begin{align}
%  \mathcal{P}^{do}_X (\bar{x} ; \pi) := \left\{P^{do}_X \mid \pi(x) = \bar{x} \;\forall x \in \text{supp}(P^{do}_X)\right\}.
% \end{align}
% }
% \begin{definition}[macro intervention set]
% A \textit{macro-intervention set}, $\cJ$, is the set of macro interventions $j(\bar{x})$ for all values of $\bar{x} \in \text{supp}\left(P(\bar{X})\right)$. 
% \end{definition}
\begin{remark}
Often, only the first element of a macro-intervention is detected since the second element involves a micro quantity. This leads to ambiguity on the effect of the macro-intervention since realisations on the micro-variables are different. See the visual illustration in Figure~\ref{fig:sales_micromacro}.
\end{remark}

% \begin{proposition}\label{ex:violate_rw17}
% Let $M\defeq (S, \cI, \mathbb{P}_{E})$ be an SEM defined in \citep{Rubenstein2017}, with
% \begin{align}
%     S &= \bigg\{ Y_1 \defeq \alpha_1 X_1, \;
%     Y_2 \defeq \alpha_2 X_2, \nonumber \bigg\} \;\;\text{where $\alpha_1 \neq \alpha_2$.}\\
%     \cI &= \bigg\{ \emptyset, do(X_1 \defeq 0, X_2 \defeq 1), do(X_1\defeq 1, X_2\defeq 0) \bigg\}. \nonumber
% \end{align}
% and $(X_1, X_2) \in \{0,1\}\times \{0,1\}$ with  $(X_1, X_2) \sim \mathbb{P}_E  \; \text{where } supp[\mathbb{P}_E] = \{0,1\}\times \{0,1\}$.

% Moreover, let $\bar{M} \defeq (\bar{S}, \bar{\cI}, \bar{\mathbb{P}}_E)$ be another SEM, with 
% \begin{align}
%     \bar{S} &= \{\bar{Y} \defeq f(\bar{X})\} \;\;\text{for some $f$,}\nonumber \\
%     \bar{\cI} &= \bigg\{\emptyset, do(\bar{X}\defeq 1)\bigg\}.
% \end{align}
% and $\bar{X} \in \{1\}, $ with $\bar{X} \sim \bar{\mathbb{P}}_E  \; \text{where } supp[\mathbb{P}_E] = \{1\}.$

% Fix the map $\tau: \cX_1 \times \cX_2 \times \cY_1 \times \cY_2 \rightarrow \bar{\cX} \times \bar{\cY}$ to be $\tau((x_1,x_2,y_1,y_2)) = (x_1+x_2,y_1+y_2)$. Then there exists no $f$ and $\omega : \cI \rightarrow \bar{\cI}$ such that $\bar{M}$ is an exact $\tau$-transformation with $M$. 
% \end{proposition}


\begin{figure*}[t]
\begin{minipage}{.45\textwidth}
    \centering
	\begin{tikzpicture}[roundnode/.style={circle, draw=black!100, fill=black!15, very thick, minimum size=0.5mm}, normalnode/.style={circle, draw=black!0, very thick, minimum size=0.5mm}, unfillednode/.style={circle, draw=black!100, very thick, minimum size=0.5mm}, squarednode/.style={rectangle, draw=red!60, fill=red!5, very thick, minimum size=5mm}, arrowhead/.style={Triangle[length=3mm, width=2mm]}]
		\node[text width=6cm, text=blue] at (3.4, 3.2) {$M$};
	    \node[text width=3cm, font = {\small}] at (0.7, 2.2) {$\bigg\{X_i \sim P_i\bigg\}_{i=1,\cdots, N}$};
		\node[unfillednode] (x1) at (-1.2,1) {$X_1$};
		\node[unfillednode] (x2) at (-1.2,0) {$X_2$};
		\node[text width=1cm] at (-0.7, -1) {$\vdots$};
		\node[unfillednode] (xN) at (-1.2,-2) {$X_N$};
		\node[unfillednode] (xbar) at (-1.2, -4) {$\bar{X}$};
		
		\node[unfillednode] (y1) at (2.2,1) {$Y_1$};
		\node[unfillednode] (y2) at (2.2,0) {$Y_2$};
		\node[text width=1cm] at (2.6, -1) {$\vdots$};
		\node[unfillednode] (yN) at (2.2,-2) {$Y_N$};
		\node[unfillednode] (ybar) at (2.2, -4) {$\bar{Y}$};
		

		
		\draw[-{Triangle[length=3mm, width=2mm]}, line width=1pt] (x1) -- node[font = {\small}, above=3pt]{$f_1(x_1) = \alpha_1 x_1$} (y1);
		\draw[-{Triangle[length=3mm, width=2mm]}, line width=1pt] (x2) -- node[font = {\small}, above=3pt]{$f_2(x_2) = \alpha_2 x_2$} (y2);
		\draw[-{Triangle[length=3mm, width=2mm]}, line width=1pt] (xN) -- node[font = {\small}, above=3pt]{$f_N(x_N) = \alpha_N x_N$} (yN);
		
		\draw[blue, thick, rounded corners=5pt]
  (-2.3,-2.8) rectangle ++(5.7,5.7);
  		\draw[dashed, thick, rounded corners=5pt]
  (-2,-2.6) rectangle ++(1.3,4.2);
    	\draw[dashed, thick, rounded corners=5pt]
  (1.7,-2.6) rectangle ++(1.3,4.2);
        \draw[{Triangle[open, length=2mm, width=2mm]}-{Triangle[open, length=2mm, width=2mm]}, line width=1pt] (-1.2, -2.6) -- node[font = {\small}, left=2pt]{$\pi$} (xbar);
        \draw[{Triangle[open, length=2mm, width=2mm]}-{Triangle[open, length=2mm, width=2mm]}, line width=1pt] (2.2, -2.6) -- node[font = {\small}, right=2pt]{$\pi$} (ybar);

	\end{tikzpicture}
\end{minipage}
\begin{minipage}{.45\textwidth}
      \centering
    \centering
	\begin{tikzpicture}[roundnode/.style={circle, draw=black!100, fill=black!15, very thick, minimum size=0.5mm}, normalnode/.style={circle, draw=black!0, very thick, minimum size=0.5mm}, unfillednode/.style={circle, draw=black!100, very thick, minimum size=0.5mm}, squarednode/.style={rectangle, draw=red!60, fill=red!5, very thick, minimum size=5mm}, arrowhead/.style={Triangle[length=3mm, width=2mm]}]
		\node[text width=6cm, text=blue] at (3.4, 3.2) {$M^{X\sim P^{do}_{\mathbf{X}|\bar{x}}}$};
	    \node[text width=3cm, text=red, font = {\small}] at (1, 2.2) {$\bigg\{\mathbf{X} \sim P^{do}_{\mathbf{X}|\bar{x}}\bigg\}$};
		\node[unfillednode] (x1) at (-1.2,1) {$X_1$};
		\node[unfillednode] (x2) at (-1.2,0) {$X_2$};
		\node[text width=1cm] at (-0.7, -1) {$\vdots$};
		\node[unfillednode] (xN) at (-1.2,-2) {$X_N$};
		\node[unfillednode] (xbar) at (-1.2, -4) {$\color{red}\bar{x}$};
		
		\node[unfillednode] (y1) at (2.2,1) {$Y_1$};
		\node[unfillednode] (y2) at (2.2,0) {$Y_2$};
		\node[text width=1cm] at (2.6, -1) {$\vdots$};
		\node[unfillednode] (yN) at (2.2,-2) {$Y_N$};
		\node[unfillednode] (ybar) at (2.2, -4) {$\bar{Y}$};
		
		
		\draw[-{Triangle[length=3mm, width=2mm]}, line width=1pt] (x1) -- node[font = {\small}, above=3pt]{$f_1(x_1) = \alpha_1 x_1$} (y1);
		\draw[-{Triangle[length=3mm, width=2mm]}, line width=1pt] (x2) -- node[font = {\small}, above=3pt]{$f_2(x_2) = \alpha_2 x_2$} (y2);
		\draw[-{Triangle[length=3mm, width=2mm]}, line width=1pt] (xN) -- node[font = {\small}, above=3pt]{$f_N(x_N) = \alpha_N x_N$} (yN);
		
		\draw[blue, thick, rounded corners=5pt]
  (-2.3,-2.8) rectangle ++(5.7,5.7);
  		\draw[dashed, thick, rounded corners=5pt]
  (-2,-2.6) rectangle ++(1.3,4.2);
    	\draw[dashed, thick, rounded corners=5pt]
  (1.7,-2.6) rectangle ++(1.3,4.2);
        % \draw[{Triangle[open, length=2mm, width=2mm]}-{Triangle[open, length=2mm, width=2mm]}, line width=1pt] (-1.2, -2.6) -- node[font = {\small}, left=2pt]{$\pi$} (xbar);
		\draw[-{Triangle[length=3mm, width=2mm]}, line width=1pt] (xbar) -- node[font = {\small}, left=2pt]{$\pi$} (-1.2, -2.6);
        \draw[{Triangle[open, length=2mm, width=2mm]}-{Triangle[open, length=2mm, width=2mm]}, line width=1pt] (2.2, -2.6) -- node[font = {\small}, right=2pt]{$\pi$} (ybar);

	\end{tikzpicture}
\end{minipage}
    \caption{\textbf{Left:} The micro-variable causal model $M$ is described by an SCM, which is shown within the blue frame. The coarsening map $\pi$ is applied to the micro-variables $X_1,\cdots, X_N$ and $Y_1, \cdots, Y_N$, both contained in the dashed frame. $\bar{X}$ and $\bar{Y}$ are the macro variables which arise from the coarsening map.
    % Note, arrows representing either the causal and coarsening relationships can all be viewed as arrows in a Bayes Net, thus give rise to conditional independence relationships. 
    \textbf{Right:} A macro-intervention $(\bar{x}, P_{\mathbf{X}|\bar{X}:=\bar{x}})$ is shown. The intervention applied to the macro variable $\bar{X}:= \bar{x}$ is realised as a (perfect) stochastic intervention on $X$, note that all values of $\mathbf{x}$ supported by $P_{\mathbf{X}|\bar{X}:=\bar{x}}$ give rise to $\bar{x}$.
\label{fig:sales_rev_micro_macro}} %\vspace*{-10mm}
\end{figure*}
% \vspace{-30em}


A macro-intervention results in a change in the causal mechanism of the micro-variables. The new micro-variable causal mechanism is given by replacing the original generative mechanism of $X$ by $P^{do}_{\pi,\bar{x}}$.


\dominik{make clear that we restrict the attention to cause-effect relations here.} 
\begin{definition}[macro-intervention graph]
Let $G^a = (\cV, \bar{\cV}, \cE, \cC)$ be an amalgamated graph. A macro intervention $\left(do(\bar{X} \defeq \bar{x}), P^{do}_{\pi, \bar{x}}\right)$ maps $G^a$ to the \textit{macro-intervention graph}, ${G^{a}}' \defeq (\cV, \bar{\cV}, \cE', \cC')$, where $\cE' = \cE \bigcup \{\bar{X} \rightarrow X\} \setminus\{V \rightarrow X : V\in \cV\setminus\{X\}\}$ and  $\cC' = \cC \setminus \{X \leftrightarrow \bar{X}\}$.
\end{definition}

Let $X$ and $Y$ be two (multi-variate) micro-variables with associated macro variables $\bar{X}$ and $\bar{Y}$. Suppose that $X$ precedes $Y$ in causal order.
Denote the pre-interventional distribution by $P$.
Given a macro intervention $j=(do(\bar{X} \defeq \bar{x}), P^{do}_{\bar{x}}(X))$, the post-intervention quantity $P^j(\bar{y}|do(\bar{X}\defeq\bar{x}))$ is well-defined: $P^j(\bar{y}|do(\bar{X}\defeq\bar{x})) = \int_{\cX, \cY} P(\bar{y}|Y=y)P(y|do(X\defeq x))P^{do}_{\pi, \bar{x}}(x) dxdy$. We can then define the notion of macro-confounding by comparing the observational and interventional distributions of macro variables. 
% \jonas{To me it seems more logical to first introduce the \textit{post-interventional distribution} $P^{do}(\bar{Y}|\bar{X})$ wrt to a given $P^{do}_{X|\bar{x}}$ and \textit{explicitly} define macro confounding wrt to a fixed macro intervention.}
\begin{definition}[macro confounding]
Let $X$ and $Y$ be two micro-variables with associated macro variables $\bar{X}$ and $\bar{Y}$; $X$ precedes $Y$ in causal order. Let $\cJ$ be a set of macro-interventions on $\bar{X}$.
We say there is $\textit{macro-confounding}$ between macro variables $\bar{Y}$ and $\bar{X}$ if $P(\bar{Y}|\bar{X}=\bar{x}) \neq P^j(\bar{Y}|do(\bar{X}\defeq \bar{x}))$ for some $j \in \cJ$.
\end{definition}
\dominik{I'm confused: I though confoundedness refers to specific $j$?} 


\begin{definition}[confounding-inducing and confounding-inhibiting implementation of interventions] 
% \dominik{is confounding-inhibiting the best term? Maybe we can talk about 'confounding-avoiding' and 'confounding-inducing' interventions. Maybe there are even better terms. When there is micro-confounding we may talk about 'confounding-breaking' versus 'confounding-preserving'?}
A \textit{confounding-inhibiting macro intervention} is a macro intervention $j$ such that the post-interventional distribution $P^j(\bar{Y}|do(\bar{X}\defeq\bar{x}))$ is equal to the observational distribution $P(\bar{Y}|\bar{X}=\bar{x})$. On the other hand, a \textit{confounding-inducing implementation} is one such that $P^j(\bar{Y}|do(\bar{X}\defeq \bar{x})) \neq P(\bar{Y}|\bar{X}=\bar{x})$.
\end{definition}


% When do confounding-inhibiting macro interventions exist? We first show an expected result: in an unconfounded micro variable model, confounding-inhibiting macro interventions always exist. However, there also exist macro interventions which would promote a sense of confounding in the macro-variable model.

\begin{thm}\label{thm:main} 
Let $X\to Y$ and $\bar{X}$ and $\bar{Y}$ be coarse-grainings of $X$ and $Y$, respectively. Then the macro-intervention
$(do(\bar{X} \defeq \bar{x}), P(X|\bar{X} \defeq \bar{x}))$ is confounding-inhibiting, that is,
the uncounfounded cause-effect relation $\bar{X} \to \bar{Y}$ 
correctly predicts the effect of interventions on $\bar{X}$. 
\end{thm}
To keep notation simple our proofs will henceforth consider discrete variables but the generalization for continuous distributions is obvious. 
\begin{proof}
$P(\bar{Y}|do(\bar{x}))= \sum_x 
P(\bar{Y}|x)P(x|\bar{x})= P(\bar{Y}|\bar{x})$.
\end{proof}
Despite its mathematical triviality, this result shows an option to define a general way of coarse-graining cause-effect relations provided one is willing to accept its  {\it context dependence}: the relation  $\bar{X} \to \bar{Y}$  
holds whenever one assumes that the implementation of $do(\bar{x})$ was done with the same conditional distribution of micro states $x$ as it is usual `in the wild'. This view, however, entails that we refer to different implementations in different 
environments in which  macro states come with different distributions of micro states. 
One may think that this context dependence comes with paradoxes. 
Let us therefore describe a slightly more involved scenario where our coarse-graining of interventions still makes sense:
consider the chain $X\to Y\to Z$, with aggregated variables $\bar{X},\bar{Y},\bar{Z}$. 
If we now define an implementation of $do(\bar{y})$, would we then define the `usual distribution' of microstates as
$P(Y|\bar{y})$ or $P(Y|\bar{x},\bar{x})$?  \yuchen{@Dominik, the preceding sentence does not make sense. Please check it.} \dominik{rephrased it slightly, please check} We could find justification for both: to someone for whom $\bar{X}$ is unobserved, the former is the usual distribution, but for someone who accounts for  $\bar{X}$, the latter is usual.  
The latter would also appear as the right one for someone who just analyzes a sub population defined by fixed $\bar{x}$.
We now observe:

\begin{lemma}\label{lem:chain} 
Given the causal chain $X\to Y\to Z$, then implementing $do(\bar{y})$ according to $P(Y|\bar{y})$ results in the same
downstream effect on $\bar{Z}$ as implementing it according to  $P(Y|\bar{y},\bar{x})$ if and only if  
\begin{equation}\label{eq:chain} 
\bar{X} \indep \bar{Z} \,|\bar{Y}.   
\end{equation} 
\end{lemma} 
\dominik{notation needs to be adapted here (use pair notation for do)} 
\begin{proof}
Implementing $do(\bar{y})$ according to $P(Y|\bar{y})$ results in the downstream effect
$\sum_y P(\bar{Z}|y)P(y|\bar{y})= \sum_y P(\bar{Z}|y,\bar{y})P(y|\bar{y}) = P(\bar{Z}|\bar{y})$. Implementation via $P(Y|\bar{y},\bar{x})$ results in $\sum_y P(\bar{Z}|y)P(y|\bar{y},\bar{x}) =\sum_y P(\bar{Z}|y, \bar{y},\bar{x})P(y|\bar{y},\bar{x})= P(\bar{Z}|\bar{y},\bar{x})$.  
The statement $P(\bar{Z}|\bar{y}) =  P(\bar{Z}|\bar{y},\bar{x})$ holds for all $\bar{x},\bar{y}$ if and only if \eqref{eq:chain}  holds. 
\end{proof}  

Note that \eqref{eq:chain} is a necessary condition for $\bar{X}\to \bar{Y}\to \bar{Z}$ to be a valid coarse graining, otherwise we would 
need to add a direct link  $\bar{X}\to \bar{Z}$, which renders
the causal relation $\bar{Y}to \bar{Z}$ confounded. 
Lemma \ref{lem:chain} thus states that choosing $P(Y|\bar{y})$
or $P(Y|\bar{y},\bar{y})$ does not matter whenever the chain can be coarse grained to a chain of macro variables.
 

\subsection{Backdoor adjustment with aggregated variables} 

Assume now we have the DAG in Figure \ref{fig:XYZ}.
\begin{figure}[t]
\resizebox{0.4\textwidth}{!}{%
	\begin{tikzpicture}[roundnode/.style={circle, draw=black!100, very thick, minimum size=0.5mm}, greynode/.style={circle, draw=black!100, fill=black!15, very thick, minimum size=0.5mm}, normalnode/.style={circle, draw=black!0, very thick, minimum size=0.5mm}, squarednode/.style={rectangle, draw=red!60, fill=red!5, very thick, minimum size=5mm}, arrowhead/.style={Triangle[length=3mm, width=2mm]}]
	    \node[roundnode] (x) at (0.5, 3) {$X$};
		\node[roundnode] (y) at (-0.8,1) {$Y$};
		\node[roundnode] (ybar) at (-0.8, -1) {$\bar{Y}$};
		\node[roundnode] (z) at (1.8, 1) {$Z$};
		\node[roundnode] (zbar) at (1.8, -1) {$\bar{Z}$};
        \node[roundnode] (xbar) at (0.5, 0) {$\bar{X}$};  
		
		\draw[-{Triangle[length=3mm, width=2mm]}, line width=1pt] (x) -- (y);
         \draw[-{Triangle[length=3mm, width=2mm]}, line width=1pt] (x) -- (z);
		\draw[{Triangle[open, length=2mm, width=2mm]}-{Triangle[open, length=2mm, width=2mm]}, line width=1pt] (y) -- node[font = {\small}, left=2pt]{$\pi_Y$} (ybar);
		\draw[{Triangle[open, length=2mm, width=2mm]}-{Triangle[open, length=2mm, width=2mm]}, line width=1pt] (z) -- node[font = {\small}, right=2pt]{$\pi_Z$} (zbar);
		\draw[-{Triangle[length=3mm, width=2mm]}, line width=1pt] (y) -- (z);
        \draw[{Triangle[open, length=2mm, width=2mm]}-{Triangle[open, length=2mm, width=2mm]}, line width=1pt] (x) -- node[font = {\small}, left=0pt]{$\pi_X$} (xbar);

    	\end{tikzpicture}
     }
     \hspace{0.3cm} 
\resizebox{0.4\textwidth}{!}{%
	\begin{tikzpicture}[roundnode/.style={circle, draw=black!100, very thick, minimum size=0.5mm}, greynode/.style={circle, draw=black!100, fill=black!15, very thick, minimum size=0.5mm}, normalnode/.style={circle, draw=black!0, very thick, minimum size=0.5mm}, squarednode/.style={rectangle, draw=red!60, fill=red!5, very thick, minimum size=5mm}, arrowhead/.style={Triangle[length=3mm, width=2mm]}]
	    \node[roundnode] (xbar) at (0.5, 3) {$\bar{X}$};
		\node[roundnode] (ybar) at (-0.8,1) {$\bar{Y}$};
%		\node[roundnode] (ybar) at (-0.8, -1) {$\bar{Y}$};
		\node[roundnode] (zbar) at (1.8, 1) {$\bar{Z}$};
%		\node[roundnode] (zbar) at (1.8, -1) {$\bar{Z}$};
		
		\draw[-{Triangle[length=3mm, width=2mm]}, line width=1pt] (xbar) -- (ybar);
         \draw[-{Triangle[length=3mm, width=2mm]}, line width=1pt] (xbar) -- (zbar);
%		\draw[{Triangle[open, length=2mm, width=2mm]}-{Triangle[open, length=2mm, width=2mm]}, line width=1pt] (y) -- node[font = {\small}, left=2pt]{$\pi_Y$} (ybar);
%		\draw[{Triangle[open, length=2mm, width=2mm]}-{Triangle[open, length=2mm, width=2mm]}, line width=1pt] (z) -- node[font = {\small}, right=2pt]{$\pi_Z$} (zbar);
		\draw[-{Triangle[length=3mm, width=2mm]}, line width=1pt] (ybar) -- (zbar);
%		\draw[-{Triangle[length=3mm, width=2mm]}, line width=1pt] (y) 
    	\end{tikzpicture}
     }
    \caption{Left: complete DAG with micro variables $X,Y,Z$, together with its aggregations $\bar{X},\bar{Y},\bar{Z}$. Right: The coarse-grained DAG which we would like to give a causal semantics by introducing appropriate interventions, if possible.}
    \label{fig:XYZ}
\end{figure}
Under which conditions can we define implementations of macro interventions with respect to which the system behaves 
like the DAG on the right of Figure \ref{fig:XYZ}? We already know that implementing $do(\bar{x})$ via $P(X|\bar{x})$
yields effects on $\bar{Y},\bar{Z}$ that align with the observational conditionals $P(\bar{Y}|\bar{X})$ and $P(\bar{Z}|\bar{X})$}, respectively. The questionable part is the effect of interventions on $\bar{Y}$. We need to define them in a way that ensures
\begin{align}\label{eq:backdoor}  
P(\bar{Z}| do(\bar{y}), \bar{x}) =  P(\bar{Z}| \bar{y}, \bar{x}), 
\end{align} 
that is, the backdoor adjustment formula with $\bar{X}$ as backdoor variable. We find the following sufficient condition:

\begin{lemma}[macro backdoor adjustment ]\label{lem:backdoor} 
Given the DAG Figure \ref{fig:XYZ}, left, let $\bar{Z}_y$ denote the random variable
$\bar{Z}$ after adjusting $Y$ to some fixed $y$ 
in the SCM for $\bar{Z}$. 
If 
\begin{equation}\label{eq:back} 
\bar{Z}_y \indep Y \,| \bar{X}, 
\end{equation} 
%Let $\bar{Z} \indep X \,| \bar{X},Y$, 
then 
\eqref{eq:backdoor} holds if $do(\bar{y})$ is defined by
randomizing $Y$ according to $P(Y|\bar{y},\bar{x})$.
\end{lemma}
\begin{proof}
For fixed $\bar{x}$, \eqref{eq:back} states that $\bar{Z}$ 
is a function of noise that is independent of
$Y$, thus we have equality of the
interventional and observational probabilities 
$
p(\bar{Z}|do(y),\bar{x}) = p(\bar{Z}|y,\bar{x}).    
$
We conclude 
$
p(\bar{Z}|do(\bar{y}),\bar{x}) = \sum_y  p(\bar{Z}|do(y),\bar{x}) p(y|\bar{y},\bar{x})
= \sum_y p(\bar{Z}|y,\bar{x}) p(y|\bar{y},\bar{x}) = p(\bar{Z}|\bar{y},\bar{x}). 
$
%For any fixed $y$ we have
%\begin{align} 
%P(\bar{Z}| do(y), \bar{x})  &= \sum_x P(\bar{Z}| y, \bar{x}, x) P(x|\bar{x}) \\ &=   P(\bar{Z}| y, \bar{x}) \sum_x P(x|\bar{x}) =   P(\bar{Z}| y, \bar{x}). 
%\end{align} 
%Hence we obtain
%\begin{align*} 
%P(\bar{Z}| do(\bar{y}), \bar{x}) &=  \sum_y P(\bar{Z}| do(y), \bar{x}) P(y| \bar{y},\bar{x}) \\
%&= \sum_y P(\bar{Z}| y, \bar{x}) P(Y| \bar{y},\bar{x}) =
%P(\bar{Z}| \bar{y}, \bar{x}). 
%\end{align*} 
\end{proof} 

Lemma \ref{lem:backdoor} states that we can consider the DAG in Figure \ref{fig:XYZ}, right as a valid coarse-graining of the one on the right when we implement $do(\bar{y})$ via $P(Y|\bar{y},\bar{x})$, provided that $\bar{X}$ blocks the backdoor path between 
$Y$ and $\bar{Z}$. 



We proceed now to analyse confounding in unconfounded micro-variable models. We focus on structural equation models with additive noise, and leave further generalisation to future work.



\section{Confounding in unconfounded micro variable models}\label{sec:unconfounded}
\vspace{-1ex}
\subsection{Toy example} \label{subsec:aggre}
\vspace{-1ex}
To consider a toy scenario in real life which matches Example \ref{ex:violate_rw17}, 
suppose there are two identical shops, $A$ and $B$, each with two products, indexed $1$ and $2$, with prices $\alpha_1$ and $\alpha_2$, respectively. The sales $X_1,X_2$ of the two products are assumed to be independent Gaussians with means
$\mu_1,\mu_2$
 and variances $\sigma_1^2,\sigma_2^2$.
%\begin{align}
%    &X_1 \sim \cN (\mu_1, \sigma_1^2) \label{eq:xa}\\
%    &X_2 \sim \cN (\mu_2, \sigma_2^2) \label{eq:xb}\\
%    &{\rm Cov}(X_1,X_2) = 0 %\label{eq:xaindepxb}
%\end{align}
The total revenue, $\bar{Y}$ is given by $\bar{Y} = \alpha_1 X_1 + \alpha_2 X_2$. Now suppose the shop owners want to understand how total revenue changes wrt total sales, $\bar{X} = X_1 + X_2$. 
%Equations \eqref{eq:xa} to \eqref{eq:xaindepxb} induce a joint distribution over $X_1$, $X_2$, $\bar{X}$ and $\bar{Y}$; denote this $P(X_1,X_2,\bar{X}, \bar{Y})$.

Shop $A$ owner performs an experiment where they set the total sales to $\bar{x}$, but in a way that respects $P$, i.e. $P^{do}(X_1,X_2|\bar{x}) \defeq P(X_1,X_2|\bar{x}})$. Clearly this leads them to conclude that $\bar{X}$ is unconfounded with due to Theorem \ref{thm:main}. 
%because 
%\vspace{-1ex}
%\begin{align}
%    P(\bar{Y}|\bar{X}) = &\int_{\cX_1, \cX_2} P(\bar{Y}|x_1,x_2) 
    % \nonumber \\
%    \cdot P(x_1, x_2|\bar{X}) dx_1 dx_2 \label{eq:sec3_toy_7}\\
%    = &\int_{\cX_1, \cX_2} P^{do}(\bar{Y}|x_1,x_2) \cdot P^{do}(x_1, x_2|\bar{X}) dx_1 dx_2 \label{eq:sec3_toy_8}\\
%    = &P^{do}(\bar{Y}|\bar{X})
%\end{align}
%\vspace{-1ex}
%\eqref{eq:sec3_toy_7} uses the fact that $\bar{X} \indep \bar{Y} | \left\{X_1,X_2\right\}$, since $\bar{X}$ is a deterministic function of $X_1$ and $X_2$.
Consequentially, the first shop owner concludes on the following structural equation which is what would be obtained by regressing $\bar{Y}$ on $\bar{X}$:
\begin{align}
    \bar{Y} &= \frac{{\rm Cov}(\bar{Y}, \bar{X})}{{\rm Cov}(\bar{X}, \bar{X})}\bar{X} + N \label{eq:200}
    = \frac{\alpha_1 \sigma^2_1 + \alpha_2\sigma^2_2}{2} \bar{X} + N,
\end{align}
%\vspace{-0.5ex}
with     $N \indep \bar{X}$.  Meanwhile, shop $B$ owner performs an experiment also setting the total sales to $\bar{x}$, but they do this by observing how many items were sold for product $1$, and then turn up (or down) the advertising to make sure they sell $\bar{x} - x_1$ items for product $2$. This amounts to the macro intervention:
\vspace{-1ex}
\begin{align}
    P^{do}_{\bar{x}} (X_1, X_2) &= \cN \left(\begin{pmatrix}\mu_1 \\ \bar{x} - \mu_1\end{pmatrix}, \begin{pmatrix}\sigma_1^2 & -\sigma_1^2 \\ -\sigma_1^2 & \sigma_1^2\end{pmatrix}\right) \label{eq:toy_ex_2}
\end{align}
% \vspace{-2ex}
Shop owner 2, making this intervention, would instead conclude that the structural equation generating $\bar{Y}$ is 
\vspace{-1ex}
\begin{align}
    \bar{Y} &= \alpha_2 \bar{X} + \tilde{N}, \label{eq:201}
\end{align}
%\vspace{-2ex}
where $\tilde{N} = (\alpha_1 - \alpha_2)X_1$.

Thus, whereever $\alpha_1 \neq \alpha_2$, we have $\tilde{N} \not \indep \bar{X}$ under $P$. 

Note that equations \eqref{eq:200}and \eqref{eq:201} generate the same observational distribution $P(\bar{Y}, \bar{X})$, but they correspond to different macro-interventions on $\bar{X}$, the former being \textit{confounding-inhibiting} while the latter being \textit{confounding-inducing}. 


% Two shop owners each sell two identical products. Denote the number of sales for each product by $X_i, i=1,\cdots, 4$. Let $P_i$ be the probability distribution of $X_i$. Each product has a fixed price, $\alpha_i$. Thus, the revenue generated from the sales of each product, denoted by $Y_i$, is given by $Y_i=\alpha_i X_i$. Moreover, the shop owners also keep track of the number of total sales and total revenue, denoted by $\bar{X} \defeq \sum_i X_i$ and $\bar{Y} \defeq \sum_i Y_i$. Assume the sales of each product of each owner is independent of each other. We represent the micro causal model and coarsening map in Figure~\ref{fig:sales_rev_micro_macro}. Now, they both want to see how the total revenue responds to an intervention on total sales. The first shop owner makes a macro intervention of setting $\bar{X}\defeq \bar{x}$, and they achieve this by setting the sale of each individual product to be $\frac{\bar{x}}{4}$. In our framework, the first shop owner had made a macro intervention $(\;\bar{x}, \prod_{i=1}^4\delta(X_i - \frac{\bar{x}}{4}))$. Meanwhile, the second shop owner also performs a macro intervention setting the total sales to be $\bar{x}$, but they achieve this by setting the sale of the individual products to have a distribution equal to the observational distribution, i.e. $P^{do}_{X|\;\bar{x}} \defeq P_{X|\;\bar{x}}$. Clearly, for the second shop owner, the observational and interventional distributions of $\bar{Y}|\bar{X}$ are the same: $P^{do}_{\bar{Y}|\bar{X}} = P_{\bar{Y}|\bar{X}}$. Thus, the second owner made a \textit{confounding-inhibiting macro intervention} with respect to which the macro variables are not confounded. For the first owner, the post-interventional distribution, $P^{do}_{\bar{Y}|\bar{X}}$ is $\delta(\bar{Y} - \frac{\bar{X}}{4}(\alpha_1+\cdots+\alpha_4))$, which is generally not the same as the observational distribution. Thus, the first owner made a macro-intervention with respect to which the macro variables are confounded. \dominik{this claim should be backed up by telling the reader what the confounder is} \yuchen{I see what you mean, but there isn't a concrete confounder variable; the confounder just comes from the micro-mechanism.}
% \dominik{I know, but we should introduce a second coarse-grained variables that acts as the confounder} 

%\begin{remark}
%As illustrated above, it is always possible to make a confounding-inhibiting macro-intervention by taking $P^{do}(X|\bar{x}) = P(X|\bar{x})$.
%\end{remark}
% \paragraph{A natural confounding-inhibiting macro-intervention.} One can always make a natural confounding-inhibiting macro-intervention to promote unconfoundedness in the macro-variables, namely $(\bar{x}, P_{X|\bar{x}})$. 
\vspace{-2ex}
\subsection{A perspective from linear change of coordinates}
\vspace{-1ex}
The above example can also be formalised by thinking of the micro variables $\mathbf{X} = X_1,\cdots, X_N$ as a coordinate system and the aggregation as a result of a linear change of coordinates. Let $H: \R^N \rightarrow \R^N$ be a bijective linear map (i.e. the change-of-coordinate map).  Further, requiring the first row of $H$ to be ones would give us the sum aggregation: 
\begin{align}
    H_{1,:}=(1,1,\dots,1) \label{eq:H_1j}
\end{align}
Then, trivially it follows that
\begin{align}\label{eq:decomp}
    \bar{Y} &\defeq \boldsymbol{\alpha}^\top \mathbf{X}\\
    &=\boldsymbol{\alpha}^\top H^{-1} H \mathbf{X}\\
    &= \underbrace{\sum_{i=1}^N \alpha_i H^{-1}_{i,1}}_{\beta} \bar{X} + \underbrace{\sum_{i, k=1}^N\sum_{j=2}^N\alpha_{i}H^{-1}_{i, j}H_{j,k}X_k}_{\bar{U}_{\beta}} \label{eq:Ybar_new_coord}
\end{align}
%\vspace{-1ex}
Therefore, after a linear change of coordinates with $\bar{X}$ being part of the new coordinate system, $\bar{Y}$ still admits a linear structural equation under the new coordinates. We can view this as a usual structural equation of $\bar{Y}$, since all we did was changing the coordinates. Now, an intervention on $\bar{X}$ amounts to changing $\bar{X}$ while not affecting remaining coordinates $\sum_{k=1}^N H_{2:, k}X_k$, and hence the noise term, $\bar{U}_{\beta}$, which is a linear combination thereof.


One may ask, since $H$ is constrained - it must satisfy \eqref{eq:H_1j} - it needs to be shown that there exist $H$ so that a given $\beta$ can be obtained. With a little bit more effort, we can also show that for any $\boldsymbol{\Delta}$ such that $\sum_{i}\Delta_i = 1$, there also exist $H$ such that $\boldsymbol{\Delta} = H^{-1}_{:, 1}$. Indeed, we check this in the following lemma. 

\begin{lemma}\label{lemma:beta_obtain}
For a given $\boldsymbol{\alpha} \in \R^N, \; \boldsymbol{\alpha}\not \propto (1,\cdots, 1)$ and $c \in \R$, there exists an invertible $N\times N$ matrix $H \in \R^{N\times N}$ such that $H_{1,i} = 1 \; \forall i=1,\cdots, N$ and $\sum_{i}\alpha_i H^{-1}_{i, 1} = c$. Moreover, for any $\boldsymbol{\Delta}$ such that $\sum_{i}\Delta_i = 1$, there also exist $H$ such that $\boldsymbol{\Delta} = H^{-1}_{:, 1}$.
\end{lemma}
The proof is in Appendix~\ref{app:aux}. Lemma~\ref{lemma:beta_obtain} shows that for any $\beta$, there exist a corresponding change-of-coordinate matrix $H$. This is remarkable: When $\beta = \frac{\text{Cov}(\bar{Y}\bar{X})}{\text{Cov}(\bar{X}, \bar{X})}$, we have $\text{Cov}(\bar{U}_{\beta}, \bar{X}) = 0$ i.e. $\bar{X}$ and $\bar{Y}$ in this case look unconfounded. On the contrary, note that $\bar{U}_{\beta} = \boldsymbol{\alpha}^\top X - \beta \bar{X}$. Therefore, as $\beta \rightarrow \infty$, $|{\rm Cov}(\bar{X}, \bar{U}_{\beta})| \rightarrow \infty$. This means that depending on the change-of-coordinate matrix chosen, $\bar{X}$ can look either unconfounded or arbitrarily strongly confounded with $\bar{Y}$. 
\vspace{-2ex}



\subsection{A Practical Construction Using Shift Interventions}
\vspace{-2ex}
In practical scenarios, it may be difficult to implement the stochastic component in the macro interventions we defined. Using a different class of interventions, known as \textit{shift interventions} \citep{rothenhaeusler:2015:shift-intervention, pmlr-v124-sani20a}, we are able to define deterministic shifts on macro variables in terms of deterministic shifts on micro variables. 

We focus on additive shift-interventions by a constant addition, $X \mapsto X+\delta$, which is a special case of general shift-interventions $X \mapsto f(X)$. Henceforth, when we refer to shift interventions, we mean interventions of the form $X\mapsto X+\delta, \; \delta \in \R$ in the context of real-valued models. In the standard setting (i.e. without dealing with aggregation), a shift intervention is implemented as the practitioner simply observe whichever treatment the subject is about to receive, and then add a constant on top of it. In Appendix~\ref{app:shift_intervention}, we elaborate on its relations with atomic interventions.


% To implement the intervention $\bar{X} \defeq \bar{X} + \bar{\Delta}$ on the macro-variables would be to distribute $\bar{\Delta}$ among the micro-variables $X_i \mapsto X_i + \Delta_i $ such that $\sum_{i=1}^N \Delta_i = \bar{\Delta}$. 


% The shift intervention changes $\bar{Y}$
% to 
% \begin{align} 
% \bar{Y}(\Delta) = \bar{Y} +
% \alpha^\top \Delta = 
% \beta \bar{\Delta} + (\boldsymbol{\alpha} - \beta \boldsmybol{1})^\top \Delta,   
% \end{align} 
% %Although the equation holds certainly for any $\beta$, we choose the one
% %the regression coefficient in the observational distribution. 
% for any $\beta \in \R$. 
% Whenever the second summand vanishes,
% i.e. 
% \begin{align}\label{eq:betaD}  
% \boldsymbol{\alpha}^\top \Delta =
% \beta\boldymbol{1}^\top \Delta
% \end{align} 
% the system responds to the
% intervention as a linear system with
% structure coefficient $\beta$. 
% To see how \eqref{eq:betaD} is related with \eqref{eq:beta}, assume an degenerate interventional distribution whose covariance is the rank one matrix 
% $\tilde{\SX}:= \Delta \Delta^\top$. Then
%  \eqref{eq:beta} yields 
%  \[
%  \beta = \boldsymbol{\alpha}^\top \Delta /   \boldsymbol{1}^\top \Delta,
%  \]
%  in agreement with \eqref{eq:betaD}.
%  Hence, this rank one covariance 
%  with appropriate $\Delta$ defines a confounding inhibiting implementation. 


\textbf{Macro models under shift interventions.} 
Clearly, the change-of-coordinate perspective also implies, as a consequence, how to distribute the shift in $\bar{X}$ to shifts in the micro-variables $X_1,\cdots, X_N$. From \eqref{eq:Ybar_new_coord}, doing $\bar{X} \mapsto \bar{X} + 1$ amounts to doing $X \mapsto X + H^{-1}_{:, 1}$:
\begin{align}
    % \bar{Y} (\bar{X}) &= \boldsymbol{\alpha}^\top H^{-1}_{:, 1} \bar{X} + U_\beta\\
    \bar{Y} (\bar{X} + 1) &= \underbrace{\boldsymbol{\alpha}^\top H^{-1}_{:, 1} \bar{X} + U_\beta}_{\boldsymbol{\alpha}^\top X} + \boldsymbol{\alpha}^\top H^{-1}_{:, 1}\\
    &= \boldsymbol{\alpha}^\top (X + H^{-1}_{:, 1})
\end{align}
i.e. shifting by $1$ on $\bar{X}$ and shifting by $H^{-1}_{:, 1}$ on the micro-variables are the same thing!

This makes calculating $\beta$ extremely easy if you have already decided how you want to shift $X$: by Lemma~\ref{lemma:beta_obtain}, $H^{-1}_{:, 1}$ can be any vector whose elements sum to $1$. Therefore, just make sure your shift vector$\boldsymbol{\Delta}$ on $X$ has elements summing to $1$, and then the structural coefficient $\beta$ is obtained by simply doing $\beta = \boldsymbol{\alpha}^\top \Delta$.
\yuchen{-----------------I got up to here on 12/02/2023----}

% Without much more complexity, we can also generalise to have additive independent noise on the outcome models $Y_i$: $Y_i = \alpha_i X_i + V_i,\; V_i \indep X_i$:
% \vspace{-2ex}
% \begin{align}
%     &\bar{Y}(\bar{X}, \bar{U}_{\beta}, \bar{V}) \defeq \boldsymbol{\alpha}^\top \mathbf{X} + \underbrace{\sum_i V_i}_{\bar{V}}\\
%     &= \underbrace{\sum_{i=1}^N \alpha_i H^{-1}_{i,1}}_{\beta} \bar{X} + \underbrace{\sum_{i, k=1}^N\sum_{j=2}^N\alpha_{i}H^{-1}_{i, j}H_{j,k}X_k}_{\bar{U}_{\beta}} + \bar{V}\\
% % \end{align}
% % \vspace{-2em}
% % \begin{align}
%     &\resizebox{0.81\hsize}{!}{%
%     $\bar{Y}(\bar{X} + \Delta, \bar{U}_{\beta}, \bar{V}) \defeq \sum_{i=1}^N \alpha_i H^{-1}_{i,1} (\bar{X} +  \Delta)+ \bar{U}_{\beta}+ \bar{V}$%
%     }\\
%     &= \left(\sum_{i=1}^N \alpha_i H^{-1}_{i,1} \bar{X}+ \bar{U}_{\beta} \right)  +  \sum_{i=1}^N \alpha_i H^{-1}_{i,1}\Delta + \bar{V} \\
%     &= \boldsymbol{\alpha}^\top \mathbf{X} + \Delta\boldsymbol{\alpha}^\top H^{-1}_{:,1}+ \bar{V}\\
%     &= \boldsymbol{\alpha}^\top (\mathbf{X} + \Delta H^{-1}_{:,1})+ \bar{V}
% \end{align}
% % \vspace{-6ex}
% i.e. A coefficient of $\beta$ on the macro level can be obtained by distributing a shift of $+\Delta$ in $\bar{X}$ to shifts given by elements in the vector $\Delta H^{-1}_{:,1}$ in the micro level. In particular, the noise $\bar{U}_{\beta}$, which is itself a function of $\mathbf{X}$, is in fact unaffected by the shift intervention:
% \begin{align}
% &\bar{U}_{\beta}(\mathbf{X}+\Delta H^{-1}_{:,1}) \nonumber\\
%     \end{align}
%     \begin{align}
%     =&\sum_{i, k=1}^N\sum_{j=2}^N\alpha_{i}H^{-1}_{i, j}H_{j,k}(X_k + \Delta H^{-1}_{k,1})\\
%     =&\sum_{i, k=1}^N\sum_{j=2}^N\alpha_{i}H^{-1}_{i, j}H_{j,k}X_k+\Delta\sum_{i, k=1}^N\sum_{j=2}^N\alpha_{i}H^{-1}_{i, j}H_{j,k} H^{-1}_{k,1}\\
%     =& \bar{U}_{\beta} + 0
% \end{align}
% where the last equality follows since the first term is simply $\bar{U}_{\beta}$ and the last term can be checked to equal $0$. Thus, this verifies that the shift intervention on $\bar{X}$ also leaves the noise $\bar{U}_{\beta}$ unaffected.



% \subsection{Implementation-dependent structure coefficient}  


% We want to elaborate on the implications of \eqref{eq:decomp}. 
% We rewrite it as
% \begin{align}
%  \bar{Y} &\defeq  \boldsymbol{\alpha}^\top \mathbf{X} = \beta \bar{X} +  \underbrace{(\boldsymbol{\alpha}- \beta \boldsymbol{1})^\top \mathbf{X}}_{U_\beta},  
% \end{align}
% where $\boldsymbol{1}:=(1,\dots,1)$ and 
% $\beta \in \R$ is arbitrary.  
% We now argue that any $\beta$ can be interpreted as a valid structure coefficient with respect to an appropriate implementation
% of $do(\bar{x})$.  
% We have seen that the implementation $P(X|\bar{x})$ is confounding inhibiting, which corresponds to the case where $U_\beta$ is independent of $\bar{X}$. This holds when we choose $\beta$ via OLS regression, that is 
% \begin{align}\label{eq:beta} 
% \beta = Cov(\bar{X},Y)/Var(\bar{X})= \boldsymbol{1}^\top \SX  \boldsymbol{\alpha}/ \boldsymbol{1}^\top \SX \boldsymbol{1},   
% \end{align} 
% where $\SX$ denotes the covariance matrix of $X$. 

% Let us now instead choose implementations $\tilde{P}(X|\bar{x})$
% obtained from a different (interventional) distribution of $X$ with covariance matrix $\tilde{\SX}$, while the observed distribution has still covariance $\SX$.
% %We assume without loss of generality that $\SX$ and $\tilde{SX}$ have the same marginal distribution
% %$P(\bar{X})$ because we are only interested in the conditional distribution of $X$, given $\bar{x}$.

% With respect to that implementation,
% $\tilde{\beta} := \boldsymbol{1}^\top \tilde{\SX}  \boldsymbol{\alpha}/ \boldsymbol{1}^\top \tilde{\SX} \boldsymbol{1}$ 
% is the right structure coefficient. Since the cause-effect relation $\bar{X}\to \bar{Y}$ is now confounded from that perspective $\beta$ is merely the OLS regression coefficient and 
% $\beta- \tilde{\beta}$ 
% is its confounding bias. 
% %It is positive whenever the covariance between $\bar{Y}$ and $\bar{X}$ in the interventional distribution is weaker than for the observational one. 

% \dominik{I would like to put  (simplified) shift intervention part here to combine the insights with the above:}

% In practical scenarios, it may be difficult to implement the stochastic component in the macro interventions we defined. Using a different class of interventions, known as \textit{shift interventions} \citep{rothenhaeusler:2015:shift-intervention, pmlr-v124-sani20a}, we are able to define deterministic shifts on macro variables in terms of deterministic shifts on micro variables. 




\vspace{-2ex}
\subsection{Non-Gaussian and non-linear generalization} 
Now assume that 
$Y_j$ is given by
\[
Y_j = f_j(X_j) + V_j, 
\] 
where $f_j$ may be non-linear functions and
$V_j$ are noise terms, independent of $X_j$ and jointly independent.

Let us first show that there is an infinite continuum of options for a structural equation that writes $\bar{Y}$
in terms of $\bar{X}$
 together with an appropriately constructed (formal) noise term. From these options, we will later chose one that renders the causal relation between $\bar{X}$ and $\bar{Y}$ unconfounded. 

We first introduce the auxiliary variable $W:= \sum_{j=1}^N 
f_j(X_j)$ and obtain
\begin{equation}\label{eq:W}
\bar{Y} = W + \bar{V},
\end{equation}
with 
$\bar{V}:= \sum_{j=1}^N V_j$.  

Let $\psi: \R^2\to \R^2$
be a bijection that leaves the first component invariant, hat is $\psi(a,b)=(a,\psi_2(a,b))$. We then have
$\psi^{-1}(a,b)=(a,\phi(a,b))$,
where $\phi$ denotes the second component of $\psi^{-1}$. 


Let us now define an additional noise variable $M:= \psi_2(\bar{X},W)$, from which we can reconstruct 
$W$ via $W = \phi (\bar{X},M)$. We can now rewrite \eqref{eq:W} as 
\begin{equation}\label{eq:nonlinconf}
\bar{Y} = \phi(\bar{X},M) + \bar{V},
\end{equation}
with $\bar{V}$ being independent of $\bar{X}$ and $M$, but possibly dependent of $\bar{X}$. 
We can then interpret 
\eqref{eq:nonlinconf} as
the SCM of a (possibly confounded) causal relation between $\bar{X} $ and $\bar{Y}$ with vector valued noise variable $(M,\bar{V})$. 

We now show that $M$ can be chosen in a way that renders this relation unconfounded. Define 
$M$ via the conditional cumulative distribution function
\[
M(\bar{x},w):= 
P(W\leq w | \bar{X} = \bar{x}). 
\] 
Whenever the conditional distribution of $W$, given $\bar{X}$ is continuous, $M$ given $\bar{X}$ is uniformly distributed for all $\bar{x}$ and thus independent of $\bar{X}$. The function $\phi$ exists if $M(\bar{x}, \cdot)$ is invertible for all $\bar{x}$. 
With such a choice of $M$,
\eqref{eq:nonlinconf} is the SCM of an unconfounded causal relation between $\bar{X}$ and $\bar{Y}$ and an intervention that keeps $M$ constant is then confounding-inhibiting. 

The different choices of $M$ may differ with respect to interpretability and the one above that renders the relation unconfounded may not be the most interpretable one. Let us revisit the example $f_j(X_j)=\alpha_j X_j$, where $\alpha_j$ is the price per unit and $V_j:=0$. We can then define the noise $M$ by the average price $
M:= \frac{\sum_{j=1}^N \alpha_j X_j}{\sum_{j=1}^N X_j}$, 
for which we obtain the SCM $\bar{Y} = \bar{X} \cdot M$. We can then think of 
an intervention that is a  marketing campaign which increases the sales of all price segments by the same percentage and thus keeps the average price $M$ constant. 
%\subsection{There are macro-interventions for which we cannot specify a macro confounder.}\label{app:macro_confounder}
%So far we have shown that the macro variables appear confounded or not, depending on the specified macro interventions. It turns out there exist macro interventions which do not make the macro variables look unconfounded, but also do not allow for an explit construction of a macro-confounder. Due to space limitation, we elaborate on this in \ref{app:macro_confounder}.




% \paragraph{A class of confounding-inhibiting macro-interventions in unfounded Linear Gaussian models.} \yuchen{Rewrite.} Given a particular value $\bar{x}_0\in \bar{\cX}$ and a coarsening map $\pi_0$, how many macro-interventions $(\bar{x}, P^{do}_{\pi, X|\bar{x}})$ are there such that $\bar{x}=\bar{x}_0$ and $\pi = \pi_0$? Moreover, how many among them are confounding-inhibiting macro-interventions? We illustrate in the case of Linear Gaussian models that there are infinitely many macro interventions corresponding to a single macro-variable value, and that among them, confounding-inhibiting interventions can be found on a majority of dimensions.

% We begin by writing down the unconfounded Linear Gaussian micro-variable model.
% \begin{align}
%     &(X_1,\cdots, X_N) \sim \mathcal{N}(\mu, \Sigma)\\
%     \forall \; i=1,\cdots, N, \;&Y_i \defeq \alpha_i X_i
% \end{align}

% We take the summation map as the coarsening map: $\pi(\mathbf{x}) = \sum_{i=1}^N x_i$.

% Thus, the macro variables are defined as $\bar{X} = \sum_{i=1}^N X_i$ and $\bar{Y} = \sum_{i=1}^N Y_i = \sum_{i=1}^N \alpha_i X_i$. 

% Recall that a random variable is a function $\Omega \rightarrow E$, where $\Omega$ is the sample space of some probability space, and $E$ is a measurable space. The space of random variables $\Omega \rightarrow E$ is a Hilbert space, $\cH$, with the inner product $\langle X, Y \rangle_{\cH} = \mathbb{E}[XY]$. Thus $X_1,\cdots X_N$ are elements of $\cH$ and $\bar{X}, \bar{Y} \in \text{Span}\{X_1,\cdots, X_N\}$. By the Gram-Schmidt process of $\bar{Y}$ on $\mathbb{E}[\bar{X}]$ and $\bar{X} - \mathbb{E}[\bar{X}]$ we can find $U$ such that $\text{{\rm Cov}}(\bar{X}, U)= 0$ and $\bar{Y} = \beta \bar{X} + U$. The conditional variable $\bar{Y}|\bar{X}$ is given by replacing $\bar{X}$ with the constant $\bar{x}$. Now, we would like $(\bar{Y}|\bar{X}=\bar{x})_{do}$ to be such that 
% \begin{align}
%     (\bar{Y}|\bar{X}=\bar{x})_{do} &= (\bar{Y}|\bar{X}=\bar{x})_{obs} \label{eq:lgunconfound}
% \end{align}
% Note that
% \begin{align}
%     (\bar{Y}|\bar{X}=\bar{x})_{do} &= \sum_i \alpha_i (X_i|\bar{X} = \bar{x})_{do} \label{eq:do} \\
%     (\bar{Y}|\bar{X}=\bar{x})_{obs} &= \sum_i \alpha_i (X_i|\bar{X} = \bar{x})_{obs} \label{eq:obs}
% \end{align}
% So, the simplest way of achieving \eqref{eq:lgunconfound} is by setting $(X_i|\bar{X})_{do} \defeq (X_i|\bar{X})_{obs}$ for all $i = 1,\cdots, N$. For a class of solutions of $(X_i|\bar{X})_{do}$, we get by considering the difference between \eqref{eq:do} and \eqref{eq:obs} that 
% \begin{align}
%     \sum_i \alpha_i \left[(X_i|\bar{X} = \bar{x})_{obs} - (X_i|\bar{X} = \bar{x})_{do} \right] &= 0
% \end{align}
% Moreover, the requirement that $\pi(x) = \bar{x}$ for all supported $x$ requires that
% \begin{align}
%     \sum_i \left[(X_i|\bar{X} = \bar{x})_{obs} - (X_i|\bar{X} = \bar{x})_{do} \right] &= 0
% \end{align}

% \kailash{Is there a closed-form solution in terms of parameters of the micro-level causal relationship and coarsening map?}
\vspace{-2ex}

\section{Confounding in confounded micro-variable models}\label{sec:confounded}
What if the micro systems themselves are confounded? Here we first present a technical result in the context of categorical variable models: even if the underlying micro system is confounded, there can still be, at times, macro interventions which make the system look unconfounded. Moreover, even if the system remains confounded after aggregation in the effect variable (i.e. the micro-variable causes are confounded with the aggregated effect variable $\bar{Y}$), the system may still regain unconfoundedness after aggregation of the micro-variable causes. In \ref{subsec:4.2}, we also provide a discussion in the continuous variable setting, focussing on linear Gaussian models.

\subsection{Discrete confounded micro models} 
% When $X$, $Y$, $Z$ are all categorical random variables, it can be shown that. The formal proof is given in the appendix, but we outline here the moral reason that the statement should be true. 

% For the observational and interventional distributions of $\bar{Y}|\bar{X}$ to be the same, i.e. unconfoundedness in the macro variables, we can consider the decomposition of $P_{\bar{Y}|\bar{X}}$ and $P^{do}_{\bar{Y}|\bar{X}}$. Since the macro interventions, $(\;\bar{x}, P_{X|\;\bar{x}})$ for various values of $\bar{x}$, only impact the generative process for $X$ and $\bar{X}$, we can observe that all other generative mechanisms are invariant before and after the intervention.  Writing down the decomposition, we get
% \begin{align}
%     P^{do}_{\bar{Y}|\bar{X}}(y) &= \sum_{i,j} P_{\bar{Y}|x_i,z_j}(y) P^{do}_{X|\bar{X}}(x_i) P_Z(z_j) \label{eq:confound1}\\
%     P_{\bar{Y}|\bar{X}}(y) &= \sum_{i,j} P_{\bar{Y}|x_i,z_j}(y) P_{X, Z|\bar{X}}(x_i, z_j) \label{eq:confound2}
% \end{align}
% Note that we omit writing $P$ where the conditionals are invariant before and after the intervention. Unconfoundedness between $\bar{X}$ and $\bar{Y}$ thus amounts to saying that the right-hand-sides of \eqref{eq:confound1} and \eqref{eq:confound2} are the same for all values of $y$. \eqref{eq:confound1} and \eqref{eq:confound2} can be written as vectorised equations, and equality of the right-hand-side amounts to saying that, roughly speaking, the difference between $P^{do}_{X|\bar{X}} \otimes P_Z$ and $P_{X, Z|\bar{X}}$ lie in the null space of $P_{\bar{Y}|X,Z}$. Why should this be true? Morally, this is because the null space of $P_{\bar{Y}|X,Z}$ is large due to the coarsening, thus possible to contain the said difference sometimes. 
\begin{thm}\label{thm:1}
Let $X, Y, Z$ be categorical variables with $|\cX|, |\cY|, |\cZ| < \infty$. Let $G$ be the causal graph with $X\rightarrow Y$, $X\leftarrow Z \rightarrow Y$, and let $\pi_X: \cX \longrightarrow \bar{\cX}$ and $\pi_Y: \cY \longrightarrow \bar{\cY}$ denote coarsening maps. Let $G^a$ be the amalgamated graph of $G$, $\pi_X$ and $\pi_Y$, ${G^a}'$ be the macro-intervention graph for an intervention on $\bar{X}$. Let $P$ denote probability distributions satisfying the conditional independence structure given by $G^a$, and $P^{do}$ denote probability distributions satisfying the independence structure given by ${G^{a}}'$. Suppose $|\bar{\cY}| < \text{min}\left(|\cX|, |\cZ|\right)$, $|\bar{\cX}| < |\cX|$. Then for any coarsening maps $\pi_X$ and $\pi_Y$, and any family of macro interventions on $\bar{X}$: $\{(\bar{x}, P^{do}_{\pi_X, X|\bar{x}})\; |\; \bar{x} \in \bar{\cX}, \; P^{do}_{\pi_X, X|\bar{x}} \neq P_{X|\bar{X}=\bar{x}}\}$ there exist at least one $P$ such that
\begin{enumerate}
    \item $P(Y|X) \not \equiv P^{do}(Y|X)$. i.e. $X$ and $Y$ are confounded.
    \item $P(\bar{Y}|X) \not \equiv P^{do}(\bar{Y}|X)$. i.e. $X$ and $\bar{Y}$ are confounded.
    \item $P(\bar{Y}|\bar{X}=
    \bar{x}) = P^{do}(\bar{Y}|\bar{X}=
    \bar{x})$ for all $\bar{x} \in \bar{\cX}$. i.e. $\{(\bar{x}, P^{do}_{X|\bar{X}})\; |\bar{x} \in \bar{\cX}\}$ are confounding-inhibiting macro interventions.
\end{enumerate}
\end{thm}

\begin{figure}[t]
    \centering
	\begin{tikzpicture}[roundnode/.style={circle, draw=black!100, very thick, minimum size=0.5mm}, greynode/.style={circle, draw=black!100, fill=black!15, very thick, minimum size=0.5mm}, normalnode/.style={circle, draw=black!0, very thick, minimum size=0.5mm}, squarednode/.style={rectangle, draw=red!60, fill=red!5, very thick, minimum size=5mm}, arrowhead/.style={Triangle[length=3mm, width=2mm]}]
	    \node[roundnode] (z) at (0.5, 3) {$Z$};
		\node[roundnode] (x) at (-0.8,1) {$X$};
		\node[roundnode] (xbar) at (-0.8, -1) {$\bar{X}$};
		\node[roundnode] (y) at (1.8, 1) {$Y$};
		\node[roundnode] (ybar) at (1.8, -1) {$\bar{Y}$};
		
		\draw[-{Triangle[length=3mm, width=2mm]}, line width=1pt] (z) -- (x);
% 		\draw[Coarsearrow] (x) -- (xbar);
% 		\draw[>=triangle 90, ->>] (x) -- (xbar);
% 		\draw[>=triangle 90, ->>] (y) -- (ybar);
		\draw[{Triangle[open, length=2mm, width=2mm]}-{Triangle[open, length=2mm, width=2mm]}, line width=1pt] (x) -- node[font = {\small}, left=2pt]{$\pi_X$} (xbar);
		\draw[{Triangle[open, length=2mm, width=2mm]}-{Triangle[open, length=2mm, width=2mm]}, line width=1pt] (y) -- node[font = {\small}, right=2pt]{$\pi_Y$} (ybar);
		\draw[-{Triangle[length=3mm, width=2mm]}, line width=1pt] (x) -- (y);
		\draw[-{Triangle[length=3mm, width=2mm]}, line width=1pt] (z) -- (y);
% 		\draw[-{Triangle[length=3mm, width=2mm]}, line width=1pt] (x) -- (xbar);
		
	\end{tikzpicture}
    \caption{abstraction on $X$}
    \label{fig:abstraction}
\end{figure}

% Meanwhile, although this theorem shows the existence of confounding-inhibiting macro interventions, it is also true that the cases where there is a confounding-inhibiting macro intervention is of Lebesgue measure 0. 

% \begin{thm}
% Take the set-up from Theorem~\ref{thm:1}. The set of $P$ satisfying the hypothesis in Theorem~\ref{thm:1} is of Lebesgue measure 0 relative to all distributions compatible with $G^a$.
% \end{thm}
% \yuchen{proof tbc}
% The proofs are found in Appendix~\ref{app:discrete}.

% Thus, among the discrete variable models with no further assumptions, even though confounded micro-variable systems with unconfounded macro-variable systems exist, they are only a very small set and we will almost never encounter them unless we can place some conditions which limit the set.
\vspace{-4ex}
\subsection{Linear Gaussian confounded models}\label{subsec:4.2}
Here we describe the case of confounding-inhibiting macro interventions for linear Gaussian models with summation for the aggregation map. We show that confounding-inhibiting macro interventions exist provided there is enough `heterogeneity' in the parameters of the model. 

Consider the following Linear Gaussian model:
\begin{align}
    \mathbf{Z} &\sim \cN(0, \Sigma_{\bf Z})\\
    \mathbf{U} &\sim \cN(0, \Sigma_{\bf U})\\
    V &\in \cN(0, \sigma^2_V) \\
    \mathbf{X} &\defeq \mathbf{Z} + \mathbf{U}\\
    \bar{Y} &\defeq \alpha^\top \mathbf{X} + \beta^\top \mathbf{Z} + V  \\
        \mathbf{Z} &\indep \mathbf{U},\;\; (\mathbf{X},\mathbf{Z}) \indep V 
\end{align}
where $\mathbf{X}, \mathbf{Z}, \mathbf{U} \in \mathbb{R}^N$, $\bar{Y}, V \in \mathbb{R}$. 
\begin{assumption}
$\mathbf{Z}$, $\mathbf{U}$ and $V$ are not degenerate. i.e. $\sigma^2_V > 0$ and $D$, $\Sigma_{\bf U}$ positive definite.
\dominik{what is $D$?}
\end{assumption}
%The sum aggregation map is chosen for $\mathbf{X}$. 
%\begin{align}
%    \bar{X} &= \pi(\mathbf{X}) = \sum_i X_i
%\end{align}
%\vspace{-1ex}
All variables are jointly Gaussian, thus in particular there is some $\mu_{obs}(\bar{x})$ and $\sigma_{obs}^2(\bar{x})$ such that
\begin{align}
    (\bar{Y}|\bar{X}=\bar{x})_{obs} \sim \mathcal{N}(\mu_{obs}(\bar{x}), \sigma^2_{obs}(\bar{x}))
\end{align}
%\vspace{-1ex}
Now the question is whether we can choose interventions $\left\{\left(\bar{x}, P^{do}(\mathbf{X}|\bar{x})\right), \bar{x}\in \mathbb{R}\right\}$ such that $P^{do}(\bar{Y}|\bar{x}) = P(\bar{Y}|\bar{x})$ for all $\bar{x}$. To this end, we restrict the choice of $P^{do}(\mathbf{X}|\bar{x})$ to (multivariate) Gaussian densities for all $\bar{x}$, so 
\vspace{-2ex}
\begin{align}
    (\mathbf{X}|\bar{X}=\bar{x})_{do} \sim \cN(\boldsymbol{\mu}^{do}_{\bf X}(\bar{x}), \Sigma^{do}_{\bf X}(\bar{x}))
\end{align}
%vspace{-2ex}
This results in the interventional random variable 
\begin{align}
    (\bar{Y} |\bar{X} = \bar{x})_{do} = &\cN (\boldsymbol{\alpha}^\top\boldsymbol{\mu}^{do}_{\bf X}(\bar{x}), \nonumber\\
    &\boldsymbol{\alpha}^\top \Sigma^{do}_{\bf X}(\bar{x})\boldsymbol{\alpha} + \boldsymbol{\beta}^\top \Sigma_{\bf Z} \boldsymbol{\beta} + \sigma^2_V)
\end{align}
%\vspace{-1ex}
Requiring unconfoundedness between $\bar{X}$ and $\bar{Y}$ (with known causal order that $\bar{X}$ precedes $\bar{Y}$) leads to matching the mean and covariance parameters of $(\bar{Y}|\bar{X})_{do}$ and $(\bar{Y}|\bar{X})$:
\begin{align}
    \boldsymbol{\alpha}^\top\boldsymbol{\mu}^{do}_{\bf X}(\bar{x}) &= \mu_{obs}(\bar{x}) \label{eq:con1}\\
    \boldsymbol{\alpha}^\top \Sigma^{do}_{\bf X}\boldsymbol{\alpha} + \boldsymbol{\beta}^\top \Sigma_{\bf Z} \boldsymbol{\beta} + \sigma^2_V &= \sigma^2_{obs}(\bar{x}) \label{eq:con2}
\end{align}
% Moreover, by definition of macro interventions, the parameters of $({\bf X}|\bar{X})_{do}$ are required to satisfy 
% \begin{align}
%     \sum_i \mu^{do}_{\mathbf{X}, i}(\bar{x}) &= \bar{x}\label{eq:con-3}\\
%     \sum_{i,j} \Sigma^{do}_{\mathbf{X}, ij} &= 0 \label{eq:con-4}
% \end{align}

\vspace{-1ex}
Any $(\mathbf{X}|\bar{X}=\bar{x})_{do}$ under a confounding-inhibiting macro-intervention satisfy \eqref{eq:con1} - \eqref{eq:con2}.

Moreover, $P^{do}_{\pi}(\mathbf{X}|\bar{x})$ has support only in the $(N-1)$-dimensional hyperplane given by $\sum_i X_i = \bar{x}$ which leads to more restriction on $\boldsymbol{\mu}^{do}_{\mathbf{X}}(\bar{x})$ and $\Sigma^{do}_{\mathbf{X}}(\bar{x})$, namely $\sum_i \mu^{do}_{\mathbf{X}, i}(\bar{x}) = \bar{x}$ and $\sum_{ij} \Sigma^{do}_{\mathbf{X}, ij}(\bar{x}) = 0$. Analysis may be made simpler by removing these two contraints via the following argument: notice that a rotation $\mathbf{R}$ which maps $(0,\cdots,0, 1) \in \mathbb{R}^N$ to $(\frac{1}{\sqrt{N}}, \cdots, \frac{1}{\sqrt{N}}) \in \mathbb{R}^N$ followed by $\mathbf{T}(\bar{x})$, a translation \dominik{confusing to write a translation like a linear operator} by length $\bar{x}$ in the direction of $(1,\cdots, 1) \in \mathbb{R}^N$ would map the random variable with a (multivariate) Gaussian distribution supported on $\left\{\mathbf{x}\in \mathbb{R}^{N}|x_N = 0\right\}$ to another random variable with distribution function supported on $\left\{\mathbf{x}\in \mathbb{R}^{N}|\sum_n x_n = \bar{x} \right\}$. Thus the set of valid $P^{do}_{\pi}(\mathbf{X}|\bar{x})$ is given by the density functions of the Gaussian random variables 
\begin{align}
   \cG(\bar{x}) &= \begin{split}\left\{ \mathbf{a}\defeq\mathbf{T}(\bar{x})\mathbf{R}\left[\mathbf{b}; 0\right] \,\bigg|\, \mathbf{b} \sim \cN(\boldsymbol{\mu}_{N-1}, \Sigma_{N-1})\;   \right.\\ \left. s.t. \;\boldsymbol{\mu}_{N-1} \in \mathbb{R}^{N-1}, \Sigma_{N-1} \in \mathbb{R}^{(N-1)^2} \right. \\ \left. \text{ and } \mathbf{v}^\top \Sigma_{N-1}\mathbf{v} \geq 0 \; \forall \mathbf{v}\in \mathbb{R}^{N-1} \right\}\end{split}
\end{align}
\dominik{consider splitting this condition somehow, e.g. by writing everything after s.th. as separate conditions.}
A valid $P^{do}_{\pi}(\mathbf{X}|\bar{x})$ can be defined by taking the density of some $\mathbf{a} \in \cG(\bar{x})$. Hence we may rewrite conditions \eqref{eq:con1} and \eqref{eq:con2} as conditions on $\boldsymbol{\mu}_{N-1}$ and $\Sigma_{N-1}$, and the confounding-inhibiting macro-intervention on $\bar{X}$ can be constructed directly from solutions (without additional constraints) of the following two conditions:
\begin{align}
    &\boldsymbol{\alpha}^\top\mathbf{T}(\bar{x})\mathbf{R}[\boldsymbol{\mu}_{N-1}; 0] = \mu_{obs}(\bar{x}) \label{eq:con3}\\
    &\resizebox{0.81\hsize}{!}{%
    $\boldsymbol{\alpha}^\top \mathbf{R} \begin{pmatrix} \Sigma_{N-1} & 0\\0 & 0 \end{pmatrix}\mathbf{R}^\top\boldsymbol{\alpha} + \boldsymbol{\beta}^\top\Sigma_{\bf Z}\boldsymbol{\beta} + \sigma^2_V = \sigma^2_{obs}(\bar{x})$%
    } \label{eq:con4}
\end{align}
\vspace{-4ex}
\paragraph{When do \eqref{eq:con3} and \eqref{eq:con4} have solutions (in $\boldsymbol{\mu}_{N-1}$ and $\Sigma_{N-1}$)?} \eqref{eq:con3} is linear and always has a family of solutions provided $\boldsymbol{\alpha}^\top \boldsymbol{T}(\bar{x})\boldsymbol{R}$ is not degenerate in the first $(N-1)$-dimensions, i.e. $\boldsymbol{\alpha} \not \propto (1, \cdots, 1) \in \mathbb{R}^{N}$. This is also required for the existence of solution of \eqref{eq:con4}. Moreover, \eqref{eq:con4} is a bilinear form induced by $\Sigma_{N-1}$. $\Sigma_{N-1}$ is a positive semi-definite symmetric bilinear form so the necessary and sufficient condition for existence of solutions is $\sigma^2_{obs}(\bar{x}) \geq \boldsymbol{\beta}^\top\Sigma_{\bf Z}\boldsymbol{\beta} + \sigma^2_V$.
\vspace{-1ex}
\paragraph{When is $\sigma^2_{obs}(\bar{x}) \geq \boldsymbol{\beta}^\top\Sigma_{\bf Z}\boldsymbol{\beta} + \sigma^2_V$?} Since $V \indep (\mathbf{X},\mathbf{Z})$, $\sigma^2_{obs}$ is the sum of $\sigma^2_V$ and $\mathbb{V}[\boldsymbol{\alpha}^\top \mathbf{X} + \boldsymbol{\beta}^\top {\bf Z} | \bar{X}=\bar{x}]$, so we only need to check the conditions for when 
\vspace{-1ex}
\begin{align}
    \mathbb{V}[\boldsymbol{\alpha}^\top \mathbf{X} + \boldsymbol{\beta}^\top {\bf Z} | \bar{X}=\bar{x}] &\geq \boldsymbol{\beta}^\top\Sigma_{\bf Z}\boldsymbol{\beta}\label{eq:49}
\end{align}
%\vspace{-1ex}
The LHS can be transformed to the sum of variance of (linear functionals of) ${\bf Z}$ and ${\bf U}$:
\vspace{-1ex}
\begin{align}
    &\mathbb{V}[\boldsymbol{\alpha}^\top \mathbf{X} + \boldsymbol{\beta}^\top {\bf Z} | \bar{X}=\bar{x}] \nonumber \\
    = &\mathbb{V}[\boldsymbol{\alpha}^\top( {\bf Z} + {\bf U}) + \boldsymbol{\beta}^\top {\bf Z}| \bar{X}=\bar{x}] \label{eq:50}
\end{align}
%\vspace{-1ex}
It is helpful to analyse the situation around $\boldsymbol{\beta} = \mathbf{0}$. When $\boldsymbol{\beta} = \mathbf{0}$, the RHS of \eqref{eq:50} is 0 and \eqref{eq:49} is trivially satisfied. Indeed, when $\boldsymbol{\beta} = \mathbf{0}$ we are back to the case with no micro-confounding, so we expect there to be confounding-inhibiting interventions. When $\boldsymbol{\beta}\neq \mathbf{0}$, it turns out that with non-degenerate ${\bf Z}$ and $U$, the RHS of \eqref{eq:50} is never $0$. This intuitively makes sense because \textit{only} when $\boldsymbol{\beta} = \mathbf{0}$ and $\boldsymbol{\alpha} \propto (1,\cdots, 1)$, the quantity $\boldsymbol{\alpha}^\top \mathbf{X} + \boldsymbol{\beta}^\top {\bf Z}$ reduces to just $\boldsymbol{\alpha}^\top \mathbf{X} \propto \bar{X}$, which when conditioned on $\bar{X}=\bar{x}$ will be constant at $\bar{x}$. In all cases where $\boldsymbol{\beta} \neq \mathbf{0}$, we always have at least a little bit of contribution from $\boldsymbol{\beta}^\top {\bf Z}$ to keep the variance positive. This is formally verified in Proposition~\ref{prop:2} in the Appendix. Now, for a fixed $\boldsymbol{\beta} \neq \mathbf{0}$ (i.e. the RHS of \eqref{eq:49} is fixed), notice that for any direction $\boldsymbol{\alpha}$ points in, \eqref{eq:50} will eventually grow larger if we keep making the length of $\boldsymbol{\alpha}$ larger without changing its direction, so eventually \eqref{eq:49} is satisfied. Formally speaking, for every $\boldsymbol{\beta}$ and (unit-length) direction vector $\mathbf{d}$, there is some threshold $t(\mathbf{d}, \mathbf{\beta})$ such that \eqref{eq:50} is satisfied whenever $\frac{\boldsymbol{\alpha}}{\|\boldsymbol{\alpha}\|} = \mathbf{d} \text{ and } \|\boldsymbol{\alpha}\| \geq t(\mathbf{d}, \mathbf{\beta})$.



Table~\ref{tab:fixed_and_free} summarises the constants, hyperparameters, and parameters in this model.

\begin{table}[H]
    \centering
    \begin{tabular}{|c|c|}
        \hline
        Parameters & $\boldsymbol{\mu}_{N-1}, \Sigma_{N-1}$\\
        \hline
        Hyperparameters & $\Sigma_{\bf Z}$, $\Sigma_{\bf U}$, $\sigma^2_V$ $\boldsymbol{\alpha}$, $\boldsymbol{\beta}$ \\
        \hline
        Constants & $\mathbf{R}$, $\mathbf{T}$\\
        \hline
    \end{tabular}
    \caption{Constants are fixed throughout. Hyperparameters define instances of the model; we are interested in solutions to our conditions \eqref{eq:con3} and \eqref{eq:con4} in terms of the parameters within a particular model instance.}
    \label{tab:fixed_and_free}
    \vspace{-2ex}
\end{table}
\vspace{-4ex}
\paragraph{Interpretation.} If we take $X_i$ to be the number of items sold on full price and $Z_i$ to be the number of products sold on promotion. Assume that if the customer buys one item on reduced price ($\beta_i$), then they will also buy one on full price ($\alpha_i$), giving rise to the micro-level SCM $X_i \defeq Z_i$ and $Y_i \defeq \alpha_i X_i + \beta_i Z_i$. Then the above formulation asserts that the shop owner selling the items can make a confounding-inhibiting macro intervention on the total number of items sold on full price ($\bar{X}$) when full prices $\boldsymbol{\alpha}$ contain enough heterogeneity compared to the reduced prices $\boldsymbol{\beta}$ i.e.  When all prices are the same, there is not enough heterogeneity in the micro-model to blur out the confounding. On the other hand, if there is enough heterogeneity in the prices, then the shop owner may find a macro-intervention on the items sold on full prices, for which they can infer the causal effect of, by directly regressing total revenue on total items sold on full price. 
In particular, they can do despite having only confounded data of items sold on full price, reduced price, and revenues! In Appendix~\ref{sec:examples}, we provide more examples illustrating aggregation in real-world scenarios.

% \paragraph{Feasibility.} Would the shop owner be able to perform the confounding-inhibiting macro intervention when it exists? After all, performing a macro intervention requires control over the micro system, but in many cases we only need to do coarsening because we can't have full control over the micro system. It turns out that the practitioner just needs a few degrees of freedom to intervene on the micro system for them to be able to make the confounding-inhibiting macro intervention.

%\vspace{-2ex}
%\section{Related work}\label{sec:related_work}
%\vspace{-2ex}
%We provide a short summary here due to space limitations, a %longer discussion is found in Appendix~\ref{app:related work}. %\citep{Rubenstein2017} propose exact transformations, following which \citep{beckers19} propose several stronger notions of causal abstraction. By Example~\ref{ex:violate_rw17}, the condition for exact transformation is unsatisfied even in extremely simple cases. By contrast, we explore what happens when exact-transformation is not possible. In a different but related direction, \citep{Beckers2019ApproximateCA} explores how to quantify the approximation error for inexact transformation. A different but closely-related line of work is undertaken by \citep{Chalupka2016MultiLevelCS, Rischel2021CompositionalAE}, where the coarsest possible consistent coarsening is sought. Our work lies in the realm beyond the coarsest consistent partition, where macro interventions become ill-defined. Finally, our work inspires assosiation with \citep{Blom2019}, which describes a framework for modelling cyclic causal models with differential equations. In our case the dynamics between the macro and micro variables are freely customisable by the practitioner, by specifying $P^{do}_{X|\;\bar{x}}$, whereas in their case, the dynamics between the macro and micro variables are already modelled by differential equations. 

\vspace{-2ex}
\section{Conclusion}\label{sec:conclusion}
\vspace{-2ex}
We have studied systems of macro-variables which come from coarsening of finer-grained, micro-variables. We give examples to illustrate the ubiquity of such systems (Appendix~\ref{sec:examples}). We note that since the aggregation map often is decided without consideration on the micro-variable system, this can lead to ill-definedness of macro-interventinos, and in particular confoundedness. We point this out both as a warning as well as an opportunity to be exploited: e.g. by deliberately choosing the most convenient macro intervention.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \section{Introduction}

% Real world process are complex and due to the needs for communication and our inability to control the fine-grained system, practitioners often choose to work with the coarsened variables. 

% For example, if a multi-national retail company wants to reason about how its sales is impacting its revenue, it is impossible for them to reason using the sales of each individual product, as there would be millions of them. Instead, they may prefer to use aggregation of the individual-level sales to make the analysis more feasible, and more interpretable.

% However, as asserted by \citep{Rubenstein2017}, \citep{beckers19} and \citep{Beckers2019ApproximateCA}, the coarsened variables do not necessarily exhibit the same properties as the micro ones. Although they provide frameworks under which the macro- and micro-models are consistent with each other, their assumptions are strong: most of the time, the macro-model would not be consistent with the micro-model. The root of the problem is that it is only possible to come up with a consistent abstraction when the micro-intervention which correspond to the same macro-intervention also give rise to the same macro-effect, see also in \citep{Chalupka2016MultiLevelCS}. 

% This is not normally satisfied in a realistic system. If the retail company decides to increase their total sales by $X$, then there are multiple ways of achieving $X$ among the individual products. Achieving $X$ by selling $X$ number of most expensive items would increase the revenue more than selling $X$ number of cheapest items. 

% In this work we take a different angle. Instead of asking for consistency, we ask to exploit the \textit{heterogeneity} of micro-interventions that correspond to the same macro-intervention. In particular, we observe that the causal property, \textit{confoundedness}, is ambiguous in the macro-variables. If the micro-variables are unconfounded, confounding can arise from coarsening by choosing certain pairings of micro-macro intervention. Meanwhile, even if micro-variables are confounded, practitioners can actually promote a sense of unconfoundedness also by choosing certain pairings of micro-macro intervention. We make precise the preceding statements in the paper, and we view this as a provokative results which can be used to the advantage of the practitioners. For example, they may choose to use the intervention which promotes a sense of unconfoundedness. 

% \begin{figure*}[ht]
%     \begin{minipage}{0.45\textwidth}
%       \begin{center}
%         \includegraphics[scale=0.6]{figures/sales_micromacro_1.pdf}
%       \end{center}
%     \end{minipage}
%     \begin{minipage}{0.45\textwidth}
%       \begin{center}
%         \includegraphics[scale=0.6]{figures/sales_micromacro_2.pdf}
%       \end{center}
%     \end{minipage}
%     \caption{Two different ways of realising the same intervention on $\bar{X}$}
%     \label{fig:sales_micromacro}
% \end{figure*}




% \section{From macro- to micro-intervention}
% Similar to \citep{Chalupka2016MultiLevelCS}, we also start by distinguishing the micro- and macro-level causal models. The micro-level causal models we will consider are defined using the framework of Structural Causal Models following \citep{pearl09}. The macro-variables are defined based on the micro-variables based on a coarsening map. 

% \begin{definition}[coarsening map]
% A coarsening map from micro-variable $X \in \cX$ to macro-variable $\bar{X} \in \bar{\cX}$ is a surjective but non-injective function $\pi: 
% \cX \rightarrow \bar{\cX}$. We graphically represent the coarsening relationship by $X \rightarrowtail \bar{\cX}$.
% \end{definition}
% In essence, a coarsening map can be any map which merges several micro-variable values into a single macro-variable value.

% Based on the coarsening map, we follow \citep{Chalupka2016MultiLevelCS} to define a macro-level intervention via actual intervention on micro-variables. Differing from their setting, we consider stochastic intervention as well as deterministic ones, while they only consider the latter.
% \begin{definition}[macro-intervention]
% A (perfect) macro-intervention is defined with respect to a coarsening map, $\pi$. It is a tuple $\left(\bar{x}, P^{do}_{X|\;\bar{x}}\right)$, where $P^{do}_{X|\;\bar{x}}$ is distribution over $X$ characterised by $\bar{x}$ such that $\pi(x) = \bar{x}$ whenever $x$ is in the support of $P^{do}_{X|\;\bar{x}}$.
% \end{definition}
% \begin{remark}
% On the macro-level, only the first element of the macro-intervention tuple is detected since the second element involves a micro quantity. If a practitioner only possesses sensitivity at the macro-level, this leads to ambiguity on the effect of the macro-intervention. See the visual illustration in Figure~\ref{fig:sales_micromacro}.
% \end{remark}
% \begin{definition}[macro causal model]
% We write $\bar{X} \rightarrow \bar{Y}$ if there exists a macro-intervention $\left(\bar{x}, P^{do}_{X|\;\bar{x}}\right)$. 
% \end{definition}
% Note that this macro causal model can be viewed as a $\tau-\omega$ transformation defined in \citep{Rubenstein2017} from the micro-causal model, by taking the set of allowed interventions as only the set of constructed macro-interventions.

% Given a macro-intervention, we can define the notion of macro-confounding by comparing the observational and interventional distributions of macro variables. Denoting the observational distribution by $P_{obs}$, we say there is \textit{macro-confounding} between macro variables $\bar{Y}$ and $\bar{X}$ if $P(\bar{Y}|\bar{X}) = P^{do}(\bar{Y}|\bar{X})$.

% \begin{definition}[confounding-inhibiting macro intervention] An \textit{confounding-inhibiting macro intervention} $I^*$ is a macro intervention such that the post-interventional distribution $P^{do}(\bar{Y}|\bar{X})$ is equal to the observational distribution $P(\bar{Y}|\bar{X})$.
% \end{definition}

% When do confounding-inhibiting macro interventions exist? We first show an expected result: in an unconfounded micro variable model, confounding-inhibiting macro interventions always exist. However, there also exist macro interventions which would promote a sense of confounding in the macro-variable model.

% \paragraph{Can this be resolved with current approaches of causal abstraction?} No, because within the given abstraction map, the only compatible allowed micro-intervention are the trivial ones. 

% \begin{figure*}[h]
% \begin{minipage}{.45\textwidth}
%       \centering
%     \includegraphics[scale=0.7]{figures/sales_rev.pdf}
% \end{minipage}
% \begin{minipage}{.45\textwidth}
%       \centering
%     \includegraphics[scale=0.7]{figures/macro_intervention.pdf}
% \end{minipage}
% \caption{\textbf{Left:} The micro-variable causal model $M$ is described by an SCM, which is shown within the blue frame. The coarsening map $\pi$ is applied to the micro-variables $X_1,\cdots, X_4$ and $Y_1, \cdots, Y_4$, both contained in the dashed frame. $\bar{X}$ and $\bar{Y}$ are the macro variables which arise from the coarsening map. Note, arrows representing either the causal and coarsening relationships can all be viewed as arrows in a Bayes Net, thus give rise to conditional independence relationships. \textbf{Right:} A macro-intervention $(\bar{x}, P_{X|\bar{X}:=\bar{x}})$ is shown. The intervention applied to the macro variable $\bar{X}:= \bar{x}$ is realised as a (perfect) stochastic intervention on $X$, note that all values of $x$ supported by $P_{X|\bar{X}:=\bar{x}}$ give rise to $\bar{x}$.}
% \label{fig:sales_rev_micro_macro}
% \end{figure*}

% \section{confounding-inhibiting macro intervention in unconfounded micro systems}
% \paragraph{A concrete example.} Two shop owners each sell four identical products. Denote the number of sales for each product by $X_i, i=1,\cdots, 4$. Let $P_i$ be the probability distribution of $X_i$. Each product has a fixed price, $\alpha_i$. Thus, the revenue generated from the sales of each product, denoted by $Y_i$, is given by $Y_i=\alpha_i X_i$. Moreover, the shop owners also keep track of the number of total sales and total revenue, denoted by $\bar{X} \defeq \sum_i X_i$ and $\bar{Y} \defeq \sum_i Y_i$. Assume the sales of each product of each owner is independent of each other. We represent the micro causal model and coarsening map in Figure~\ref{fig:sales_rev_micro_macro}. Now, they both want to see how the total revenue responds to an intervention on total sales. We point out here a simple observation that different realisations in the micro-variables the same The first shop owner perform an experiment by setting the total sales to be $\bar{x}$ and the sale of the individual products to be the observational distribution $P(X|\bar{x})$. Meanwhile, the other shop owner also sets the total sales to be $\bar{x}$ but via setting the sale of each individual product to be $\frac{\bar{x}}{4}$. For the first shop owner, the observational and post-interventional distributions of $\bar{Y}|\bar{X}$ are the same: $P^{do}(\bar{Y}|\bar{X}) = P(\bar{Y}|\bar{X})$. Thus, the first owner made an \textit{confounding-inhibiting macro intervention} with respect to which the macro variables are not confounded. For the second owner, the post-interventional distribution, $P^{do}(\bar{Y}|\bar{X})$ is $\delta(\bar{Y} - \frac{\bar{x}}{4}(\alpha_1+\cdots+\alpha_4))$, which is generally not the same as the observational distribution. Thus, the second owner made a macro-intervention with respect to which the macro variables are confounded.
% \paragraph{A natural confounding-inhibiting macro-intervention.} Observe that in the preceding example there is no confounding between the micro cause variable $X = (X_1,\cdots, X_4)$, and the micro effect variable $Y = (Y_1,\cdots, Y_4)$. In this case, we can always make a natural confounding-inhibiting macro-intervention to promote unconfoundedness in the macro-variables, namely $(\;\bar{x}, P_{X|\;\bar{x}})$.




% \begin{remark}
% It should be pointed out that the intervention on $\bar{X}$ isn't even conceived in the natural way of using the SCM framework. First of all, one could argue that the relationship between $X_1,\cdots, X_4$ and $\bar{X}$ is constitutive and not causal. Even if one agrees to treat the relationship $\bar{X}=X_1+X_2+X_3+X_4$ as a causal relationship, one ultimately has to pick a direction for the causal assignment. The natural choice would be to say $\bar{X}\defeq X_1+X_2+X_3+X_4$. Additionally define similarly the causal relationship between the product-level revenue and total revenue, namely $\bar{Y}\defeq Y_1+Y_2+Y_3+Y_4$. Then this gives rise to the causal diagram as in Figure~\ref{fig:sales_rev}. However, according to this causal diagram, there is no causal effect from $\bar{X}$ to $\bar{Y}$, which clearly contradicts our intuition. One could instead define $X_1 \defeq \bar{X} - X_2 - X_3 - X_4$, but then the issue of the lack of product space domain arises again.
% \end{remark}
% \begin{remark}
% Can we instead model this using a cyclic causal model? \textcolor{red}{Need to think about this, but my impression is that cyclic causal models needs to use some initial conditions to fix solutions which themselves come from fixed differential equations. The differential equations determines the dynamics between the nodes. This case is different because the dynamics between the nodes is, in a sense, arbitrary up to the practitioner.}
% \end{remark}

% The above examples illustrate where the existing language of SCMs do not allow us to describe all variables on which we might be interested to understand an intervention. In particular, we explicated the different `actual' interventions which may have corresponded to the same `coarse' intervention that the practitioner is aware of. 




% % - In this section, following the introduction, I am going to illustrate the consequence of coarsening as a special case of misspecification when using Pearl's framework. 
% % - 



% \section{confounding-inhibiting macro intervention in confounded systems}
% What if the micro systems themselves are confounded? The first thing we can show is that for discrete confounded causal models, there \textit{sometimes exist} a confounding-inhibiting macro intervention. 
% \subsection{Discrete confounded micro models}
% \begin{thm}
% Let $X, Y, Z$ be categorical variables with $|\cX|, |\cY|, |\cZ| < \infty$. Let $G$ be the causal graph with $X\rightarrow Y$, $X\leftarrow Z \rightarrow Y$. Define macro variables $\bar{X}, \bar{Y}$ such that $|\bar{\cX}| < |\cX|, |\bar{\cY}| < |\cY|$. Then exists a coarsening map $\pi$, macro interventions for each value of $\bar{X}$, $\{(\bar{x}, P^{do}_{X|\;\bar{X}})\; \text{for all}\; \bar{x} \in \bar{\cX}\}$ and a micro causal model with causal graph $G$ such that 
% \begin{enumerate}
%     \item $P(Y|X) \not \equiv P^{do}{Y|X}$ i.e. $\{(\bar{x}, P^{do}_{X|\;\bar{X}})\; \text{for all}\; \bar{x} \in \bar{\cX}\}$ are confounding-inhibiting macro interventions.
%     \item $P(\bar{Y}|\bar{X}=
%     \bar{x}) \equiv P^{do}(\bar{Y}|\bar{X}=
%     \bar{x})$ for all $\bar{x} \in \bar{\cX}$.
% \end{enumerate}
% \end{thm}
% The proof is provided in the appendix. 
% \begin{figure}[t]
%     \centering
% 	\begin{tikzpicture}[roundnode/.style={circle, draw=black!100, very thick, minimum size=0.5mm}, greynode/.style={circle, draw=black!100, fill=black!15, very thick, minimum size=0.5mm}, normalnode/.style={circle, draw=black!0, very thick, minimum size=0.5mm}, squarednode/.style={rectangle, draw=red!60, fill=red!5, very thick, minimum size=5mm}, arrowhead/.style={Triangle[length=3mm, width=2mm]}]
% 	    \node[roundnode] (z) at (0.5, 3) {$Z$};
% 		\node[roundnode] (x) at (-0.8,1) {$X$};
% 		\node[roundnode] (xbar) at (-0.8, -1) {$\bar{X}$};
% 		\node[roundnode] (y) at (1.8, 1) {$Y$};
% 		\node[roundnode] (ybar) at (1.8, -1) {$\bar{Y}$};
		
% 		\draw[-{Triangle[length=3mm, width=2mm]}, line width=1pt] (z) -- (x);
% % 		\draw[Coarsearrow] (x) -- (xbar);
% 		\draw[>=triangle 90, ->>] (x) -- (xbar);
% 		\draw[>=triangle 90, ->>] (y) -- (ybar);
% 		\draw[-{Triangle[length=3mm, width=2mm]}, line width=1pt] (x) -- (y);
% 		\draw[-{Triangle[length=3mm, width=2mm]}, line width=1pt] (z) -- (y);
% % 		\draw[-{Triangle[length=3mm, width=2mm]}, line width=1pt] (x) -- (xbar);
		
% 	\end{tikzpicture}
%     \caption{abstraction on $X$}
%     \label{fig:abstraction}
% \end{figure}



% This theorem asserts that, even when the underlying micro system is itself confounded, there are still times when choosing the right macro intervention can make the macro system look unconfounded! The high-level reason of this is that due to the coarsening, the macro system can blur out the structure of the micro system, which make the confounding at the micro level invisible at the macro level. 

% Meanwhile, although this theorem shows the existence of confounding-inhibiting macro interventions, it is also true that the cases where there is a confounding-inhibiting macro intervention is of Lebesgue measure 0. 

% \begin{thm}
% Let $G$ be the causal graph with $X\rightarrow Y$, $X\leftarrow Z \rightarrow Y$. The set of distributions compatible with $G$, which satisfy
% \begin{enumerate}
%     \item $P(Y|X) \not \equiv P^{do}{Y|X}$ i.e. $\{(\bar{x}, P^{do}_{X|\;\bar{X}})\; \text{for all}\; \bar{x} \in \bar{\cX}\}$ are confounding-inhibiting macro interventions.
%     \item $P(\bar{Y}|\bar{X}=
%     \bar{x}) \equiv P^{do}(\bar{Y}|\bar{X}=
%     \bar{x})$ for all $\bar{x} \in \bar{\cX}$.
% \end{enumerate}
% is of Lebesgue measure 0 relative to all distributions compatible with $G$.
% \end{thm}

% Thus, among the discrete variable models with no further assumptions, even though confounded micro-variable systems with unconfounded macro-variable systems exist, they are only a very small set and we will almost never encounter them unless we can place some conditions which limit the set.

% \subsection{Linear Gaussian confounded models}
% In the following, we describe the case of confounding-inhibiting macro interventions for linear Gaussian models with summation coarsening map. We show that confounding-inhibiting macro interventions exist provided the variance in the parameters of the model is large enough. 

% We consider the following Linear Gaussian model:
% \begin{align}
%     Z &\sim \mathcal{N}(0, D)\\
%     X &= Z \\
%     Y &= \alpha^\top X + \beta^\top Z
% \end{align}
% where $D$ is a diagonal $N \times N$ matrix and $X, Y, Z \in \mathbb{R}^N$. We choose the following coarsening map:
% \begin{align}
%     \bar{X} &= \pi(X) = \sum_i X_i\\
%     \bar{Y} &= \pi(Y) = \sum_i Y_i
% \end{align}
% \todo[inline] {add in the justification for choosing\Sigma_{\bf Z}diagonal.}

% We will compute first the observational distribution of $\bar{Y}|\bar{X}$ and then the interventional one.

% It is known that for a multivariate Gaussian variable $X$, $X|\bar{X}$ is joint Gaussian. Write $\bar{D}_i = D_{ii}$
% \begin{align}
%     X|(\bar{X}=s) &\sim \mathcal{N}\left(\frac{s}{\sum_{i}D_{ii}}\bar{D},\Sigma_{\bf Z}- \frac{\bar{D}\bar{D}^\top}{\sum_{i}D_{ii}}\right) \\
%     (\bar{Y}|\bar{X}=s)_{obs} &\sim \mathcal{N}\left(\mu_{obs}, \sigma^2_{obs} \right)
% \end{align}
% where 
% \begin{align}
%     \mu_{obs} &= \frac{s\sum_{i}D_{ii}(\alpha_i + \beta_i)}{\sum_iD_{ii}}\\
%     \sigma^2_{obs} &= \sum_i D_{ii}(\alpha_i + \beta_i)^2 - \frac{(\sum_i D_{ii} (\alpha_i + \beta_i))^2}{\sum_i D_{ii}}
% \end{align}
% \todo[inline]{add in appendix the derivation of this.}

% Now, we wish to define a macro intervention $(\bar{x}, P^{do}_{X|\;\bar{x}})$. To do this we need to choose a $P^{do}_{X|\;\bar{x}})$ such that every value $x$ which lie in the support of $P_{X|\;\bar{x}}$ would satisfy $\pi(x) = \bar{x}$. We restrict the choices of $P^{do}_{X|\;\bar{x}})$ to Gaussian distributions. Choosing a Gaussian distribution over $\cX$ such that the sum of the components equals $\bar{x}$ amounts to choosing a Gaussian distribution in the $(N-1)$-dimensional hyperplane given by $\sum_i X_i = 
% \bar{x}$. 

% We achieve this by first choosing a Gaussian distribution in the first $(N-1)$-dimension, and then align with the hyperplane of $\sum_i X_i = 
% \bar{x}$ by a translation of $\bar{x}$ in the $N$th dimension followed by the unique rotation $R$ which maps $(0,\cdots, 0, 1) \in \mathbb{R}^N$ to $(\frac{1}{\sqrt{N}}, \cdots, \frac{1}{\sqrt{N}}) \in \mathbb{R}^N$. 

% Mathematically, this amounts to choosing $\mu_{N-1} \in \mathbb{R}^{N-1}$ and $\Sigma_{N-1} \in \mathbb{R}^{(N-1)^2}$ where $\Sigma_{-1}$ is a positive semi-definite symmetric matrix. Then define $\mu_{-1}$ 
% \begin{align}
%     \mu_{-1} &= \left(\mu_{N-1}, 0\right)\\
%     \Sigma_{-1} &= \begin{pmatrix} \Sigma_{N-1} & 0 \\ 0 & 0\end{pmatrix}
% \end{align}
% And then the chosen $P^{do}_{X|\;\bar{x}}$ is
% \begin{align}
%     P^{do}_{X|\;\bar{x}} &= \mathcal{N}(R(\mu_{-1} + \bar{x}\mu_N), R\Sigma_{-1}R^\top)
% \end{align} 
% where $\mu_N = (0,\cdots, 0, 1) \in \mathbb{R}^N$
% For clarity we state in Table~\ref{tab:fixed_and_free} the fixed and free parameters when choosing a macro intervention for the model. 
% \begin{table}[H]
%     \centering
%     \begin{tabular}{|c|c|}
%         \hline
%         Free parameters & $\mu_{N-1}, \Sigma_{N-1}$\\
%         \hline
%         Fixed parameters & $D$, $\alpha$, $\beta$, $R$, $\mu_N$ \\
%         \hline
%     \end{tabular}
%     \caption{Free and fixed parameters for the Linear Gaussian model. The free parameters can be customised when choosing a macro intervention on $\bar{X}$. Parameters which are functions of other parameters are not included.}
%     \label{tab:fixed_and_free}
% \end{table}
% For a chosen $\mu_{N-1}$ and $\Sigma_{N-1}$, the post-interventional distribution of $\bar{Y}|\;\bar{x}$ is 
% \begin{align}
%     (\bar{Y}|\;\bar{x})_{do} \sim \mathcal{N}(\alpha^\top R (\mu_{-1} + \bar{x} \mu_N), \alpha^\top R \Sigma_{-1} R^\top \alpha + \beta^\top\Sigma_{\bf Z}\beta)
% \end{align}

% For a confounding-inhibiting macro intervention, we need to choose $\mu_{N-1}$ and $\Sigma_{N-1}$ such that $(\bar{Y}|\bar{X})_{do} = (\bar{Y}|\bar{X})_{obs}$. Since both sides of the equation are Gaussian distributions, this amounts to matching both the mean and variance:
% \begin{align}
%     \alpha^\top R(\mu_{-1} + \bar{x}\mu_N) &= \mu_{obs} \label{eq:lg_con1} \\
%     \alpha^\top R \Sigma_{-1} R^\top \alpha + \beta^\top\Sigma_{\bf Z}\beta &= \sigma^2_{obs} \label{eq:lg_con2} 
% \end{align}
% Note that \eqref{eq:lg_con1} can be transformed to a linear equation of $\mu_{N-1}$, which always has a solution. Meanwhile, \eqref{eq:lg_con2} is a function of $\Sigma_{N-1}$, which only has a solution if and only if
% \begin{align}
% \sigma^2_{obs}&\geq \beta^\top\Sigma_{\bf Z}\beta \label{eq: lg_condition}
% \end{align}
% In particular, this condition implies that $\alpha + \beta$ is not a multiple of $(1,\cdots, 1)$, and needs to have a large enough component in the hyperplane perpendicular to $(1,\cdots, 1)$.
% \textcolor{red}{A detailed derivation of the above is provided in the Appendix.}

% \paragraph{Interpretation.} If we take $X_i$ to be the number of items sold on full price and $Z_i$ to be the number of products sold on promotion. Assume that if the customer buys one item on reduced price ($\beta_i$), then they will also buy one on full price ($\alpha_i$). Then the above formulation asserts that the shop owner selling the items can make a confounding-inhibiting macro intervention on the total number of items sold on full price ($\bar{X}$) when the sums of full and reduced prices for the products ($\{\alpha_i + \beta_i\}_{i=1}^N$) contain enough heterogeneity. When all prices are the same, there is not enough heterogeneity in the micro-model to blur out the confounding. On the other hand, if there is enough heterogeneity in the prices, then the shop owner may succeed to match the observational model by calibrating using the variance of the sales of the individual products. If the shop owner is able to perform the confounding-inhibiting macro intervention, then they receive an unconfounded macro causal model with respect to that intervention. This is useful because they can obtain the causal effect of that macro intervention directly from the observational distribution.

% \paragraph{Feasibility.} Would the shop owner be able to perform the confounding-inhibiting macro intervention when it exists? After all, performing a macro intervention requires control over the micro system, but in many cases we only need to do coarsening because we can't have full control over the micro system. It turns out that the practitioner just needs a few degrees of freedom to intervene on the micro system for them to be able to make the confounding-inhibiting macro intervention.

% \begin{thm}

% \end{thm}


% \section{Related work}



==> natural_interventions.tex <==
\section{When are ``natural interventions'' natural?}

Consider the following instrumental variable setting with
\[
I \to X \to Y,
\]
where $X$ and $Y$ are vectors and $I$ is a scalar. 
Whenever we have 
\[
I \independent \bar{Y} \,| \bar{X},
\]
we can consider interventions on $I$ as soft interventions on $\bar{X}$ for which
$P(\bar{Y}|do(\bar{x})=P(\bar{Y}|x)$.

It is not clear, however, whether this is a natural intervention, but it also has the property of being observation-aligning. 



==> packages.tex <==
%% Choose your variant of English; be consistent
\usepackage[american]{babel}
% \usepackage[british]{babel}

\usepackage{mathtools} % amsmath with fixes and additions
% \mathtoolsset{showonlyrefs,showmanualtags} % only show equation numbers of referenced equations

% \usepackage{siunitx} % for proper typesetting of numbers and units
\usepackage{booktabs} % commands to create good-looking tables
% \usepackage[table,xcdraw]{xcolor}

\usepackage{tikz} % nice language for creating drawings and diagrams
\usetikzlibrary{arrows.meta}
\usepackage{tikz}
\usetikzlibrary{positioning,shapes, arrows}
\tikzset{events/.style={ellipse, draw, align=center},}
% \usetikzlibrary{arrows}
% \pgfarrowsdeclarecombine{twotriang}{twotriang}%
% {triangle 90}{triangle 90}{triangle 90}{triangle 90}


%% Provided macros
% \smaller: Because the class footnote size is essentially LaTeX's \small,
%           redefining \footnotesize, we provide the original \footnotesize
%           using this macro.
%           (Use only sparingly, e.g., in drawings, as it is quite small.)

%% Self-defined macros
% \newcommand{\swap}[3][-]{#3#1#2} % just an example



% \usepackage[round]{natbib}
% \renewcommand{\bibname}{References}
% \renewcommand{\bibsection}{\subsubsection*{\bibname}}

% If you use BibTeX in apalike style, activate the following line:
% \bibliographystyle{apalike}

\usepackage{amsmath,amsthm, amssymb,mathtools}
\usepackage{rotating}
\usepackage{caption}

% \usepackage{float}
\usepackage{lineno}
\usepackage{microtype}
\usepackage{graphicx}
\usepackage{floatrow}
% \usepackage{subfigure}
\usepackage{booktabs} % for professional tables
% hyperref makes hyperlinks in the resulting PDF.
% If your build breaks (sometimes temporarily if a hyperlink spans a page)
% please comment out the following usepackage line and replace
% \usepackage{icml2020} with


\usepackage{hyperref}
\usepackage{cleveref}
\usepackage{physics}
\usepackage{algorithm, algpseudocode}
\makeatletter
\renewcommand{\ALG@name}{Algorithm}
\newcommand\StateX{\Statex\hspace{\algorithmicindent}}
\newcommand{\INDSTATE}[1][1]{\STATE\hspace{#1\algorithmicindent}}

% \newcommand{\Function}[1]{\item[]\noindent\ALG@special@indent \textbf{function:}\ #1}
% \newcommand{\EndFunction}{\item[]\noindent\ALG@special@indent \textbf{End Function}}

\makeatother
\usepackage[caption=false]{subfig} 
\usepackage{booktabs} 
\usepackage{graphicx}
\usepackage{wrapfig}
\usepackage{bbm}
 
\usepackage[utf8]{inputenc}
\usepackage{amsthm}
\usepackage[inline]{enumitem}
 
%\usepackage{subcaption}
\colorlet{myBlue}{blue!60!black}

\usepackage{soul} 
\usepackage{hyperref}
\hypersetup{ 
    colorlinks=false,
    linkcolor=blue, 
    filecolor=magenta,        
    urlcolor=myBlue,
    citecolor=cyan
}
\urlstyle{same}    
  

\usepackage{amsmath, amssymb, mathtools} 
\usepackage{cleveref} 
\crefname{assumption}{assumption}{assumptions}
\usepackage{bm}




\usepackage{lipsum}
  
% Here you can add a line with your initials to put colored remarks in margin - cf latex commands
\usepackage[textwidth=80pt]{todonotes}
% \usepackage[ruled,lined, boxed, linesnumbered,commentsnumbered,algo2e]{algorithm2e}    %AG: pass algo2e to package to remove compile errors
% \usepackage[9-41]{pagesel}

% \newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{blue}{#1}}
% \SetCommentSty{mycommfont}

% theorem style
\newtheoremstyle{styledef}
  {2pt}% space above
  {0pt}% space below
  {}%body font
  {0em}%indent amount
  {\bfseries}%Theorem head
  {}%punctuation
  {1em}%space after theorem head
  {}
\theoremstyle{styledef}



% spacing
\usepackage[font=small,skip=4pt]{caption}
% \setlength\abovecaptionskip{-5pt}

\usepackage{titlesec}
% \titlespacing*{\section}
% {0pt}{0.0ex plus .1ex minus .2ex}{0.0ex plus .2ex}
% \titlespacing*{\subsection}
% {0pt}{0.0ex plus .1ex minus .2ex}{0.0ex plus .2ex}

\input{latex_commands.tex}

\usepackage{wrapfig}
